Otimizacao e Processos Estocasticos Aplicados a Economia e Financas

Optimization and Stochastic Processes Applied to Economy and Finance -- is the name of this book translated to English; It has been used at the IME-USP - The Institute of Mathematics and Statistics of the University of Sao Paulo, since 1993. Contents: Ch.1: Linear Programming; Ch.2: Non-Linear Programming; Ch.3: Quadratic Programming; Ch.4: Markowitz Model; Ch.5: Dynamic Programming; Ch.6: LQG Estimation and Control; Ch.7: Decision Trees; Ch.8: Pension Funds; Ch.9: Mixed Portfolios Including Derivative Contracts; Appendices: App.A: Matlab; App.B: Critical-Point Software; App.C: Computational Linear Algebra; App.D: Probability; App.E: Computer Codes. This book is written in Portuguese language.

==> capref.tex <==






\chapter*{References}
\addcontentsline{toc}{chapter}{References}        
\markboth{REFERENCES}{REFERENCES} 

 \renewcommand{\baselinestretch}{0.97}
 \parskip 0.08cm
 \begin{small} 
 %\begin{footnotesize} 
 %\begin{scriptsize} 



 \r E. Aarts, J. Korst (1989).
 {\it Simulated Annealing and Boltzmann Machines}.
 Chichester: John Wiley. 

 \r K.M.Abadir, J.R.Magnus (2005).  
  {\it Matrix Algebra.}  Cambridge University Press. 

 \r J.M.Abe, B.C.Avila, J.P.A.Prado (1998). 
 {\it Multi-Agents and Inconsistence.} 
 ICCIMA'98. %131--142. 
 2nd International Conference on Computational Intelligence and 
 Multimidia Applications. Traralgon, Australia.

 \r S.Abe, Y.Okamoto (2001). {\it Nonextensive Statistical Mechanics 
 and Its Applications.} NY: Springer. 

 \r R.P.Abelson (2000). {\it Statistics as Principled Argument.} LEA. 
 
 \r P.Achinstein (1965). Theoretical Models. {\it British Journal
  for the Philosophy of Science,} 16, 102-20. 

  \r P.Achinstein (1968). {\it Concepts of Science. A Philosophical 
  Analysis.} Baltimore. 

 \r D.H. Ackley (1987).
 {\it A Connectionist Machine for Genetic Hillclimbing}.
 Boston: Kluwer.


 \r P.S.Addison (1997). {\it Fractals and Chaos: 
  An Illustrated Course.} Philadelphia: Institute of Physics. 

 \r D.Aigner, K.Lovel, P.Schnidt (1977). Formulation and Estimation 
 of Stachastic Frontier Production Function Models. {\it Journal of 
 Econometrics}, 6, 21--37. 

 \r J.Aitchison (2003). {\it The Statistical Analysis for Compositional 
 Data} (2nd edition). Caldwell: Blackburn Press. 

 \r J.Aitchison,  S.M.Shen (1980). Logistic-Normal Distributions: Some 
Properties and Uses. {\it Biometrika}, 67, 261-72. 

 \r H.Akaike (1969). Fitting Autoregressive Models for Prediction. 
 {\it Ann. Inst. Stat. Math,} 21, 243--247. 

 \r H.Akaike (1970). Statistical Prediction Identification. 
 {\it Ann. Inst. Stat. Math,} 22, 203--217.  

 \r H.Akaike (1974). A New Look at the Statistical Model 
 Identification. {\it IEEE Trans. Autom. Control.} 19, 716--723.  

 \r J.H.Albert (1985). Bayesian Estimation Methods for Incomplete
Two-Way Contingency Tables using Prior Belief of Association, in
Bayesian Statistics 2:589-602, Bernardo, JM; DeGroot, MH; Lindley, DV;
Smith, AFM eds. Amsterdam, North Holland.

 \r J.H.Albert, A.K.Gupta (1983). Bayesian Estimation Methods for 2x2
Contingency Tables using Mixtures of Dirichlet Distributions. 
 {\it JASA} 78, 831-41.

 \r R.Albright, J.Cox, D.Dulling, A.N.Langville, C.D.Meyer (2006). 
 Algorithms, Initializations, and Convergence for the Nonnegative 
 Matrix Factorization. 

 \r J.Alcantara, C.V.Damasio, L.M.Pereira (2002).
 Paraconsistent Logic Programs.  
 %WoPaLo-2002. 1st Workshop on Paraconsistent Logic. Trento, Italy. 
 JELIA-02. 8th European Conference on Logics in Artificial Intelligence. 
 {\it Lecture Notes in Computer Science,} 2424, 345--356. 

 \r G.J.Alexander and J.C.Francis. ``Portfolio Analysis.'' 
 Prentice-Hall, Englewood Cliffs, New Jersey, 1986. 

 \r G.W.Allport, H.S.Odbert (1936). Trait Names: A Psycho-Lexical
  Study. {\it Psychological Monographs}, 47, No.211. 

 \r  E.Anderson (1935). The Irises of the Gasp\'{e} Peninsula. 
 {\it Bulletin of the American Iris Society,} 59, 2-5. 

 \r T.W.Anderson (1969). {\it Statistical Inference for Covariance 
 Matrices with Linear Structure.} in Krishnaiah, P. Multivariate 
 Analysis II, NY: Academic Press. 

 \r P.Angeline. Two Self-Adaptive Crossover Operators for Genetic 
 Programming. ch.5, p.89-110 in Angeline and Kinnear (1996).

 \r P.J.Angeline, K.E.Kinnear (1996). {\it Advances in Genetic Programming.  
 Vol.2, Complex Adaptive Systems.}. MIT. 

 \r M.Anthony, N.Biggs (1992). {\it Computational Learning Theory.} 
 Cambridge Univ. Press. 

 \r M.A.Arbib, E.J.Conklin, J.C.Hill (1987).  
 {\it From Schemata Theory to Language.} Oxford University Press.  

 \r M.A.Arbib, Mary B. Hesse (1986). {\it The Construction of 
   Reality.} Cambridge University Press. 

 \r O.Arieli, A.Avron (1996).
 Reasoning with Logical Bilattices.
 {\it Journal of Logic, Language and Information}, 5, 25--63. 


 \r A.C.Atkinson (1970). A Method for Discriminating Between 
 Models. {\it J. Royal Statistical Soc. B}, 32, 323-354. 

 \r A.Aykac, C.Brumat, eds. (1977). {\it New Developments in the 
 Application of Bayesian Methods.} Amterdam: North Holland.  


 \r J.Baggott (1992). {\it The Meaning of Quantum Theory.} 
  Oxford University Press. 

 \r   L. H. Bailey (1894). Neo-Lamarckism and Neo-Darwinism.  
 {\it The American Naturalist}, 28, 332, 661-678. 

 \r  T.Bakken, T.Hernes (2002). 
 {\it Autopoietic Organization Theory. 
  Drawing on Niklas Luhmann's Social  Systems Perspective.}  
 Copenhagen Business School. %Press. 

 \r   G.van Balen (1988). The Darwinian Systhesis: A Critique of the 
   Rosenberg / Williams Argument. {\it British Journal of the 
   Philosophy of Science}, 39, 4, 441-448. 

 \r J.D.Banfield,A.E.Raftery (1993). Model Based Gaussian and 
 nonGaussian Clustering. {\it Biometrics},803-21. %49,  

 \r W.Banzahf, P.Nordin, R.E.Keller, F.D.Francone (1998). 
 {\it Genetic Algorithms.}  

 \r D.Barbieri (1992). Is Genetic Epistemology of Any Interest 
 for Semiotics? {\it Scripta Semiotica 1, 1-6.} 

 \r R.E.Barlow, F.Prochan (1981). {\it Statistical Theory of 
  Reliability and Life Testing Probability Models.} 
 Silver Spring: To Begin With.  

 \r G.A.Barnard (1947). The Meaning of Significance Level. 
 {\it Biometrika}, 34, 179--182. 

 \r G.A.Barnard (1949). Statistical Inference. 
 {J. Roy. Statist. Soc. B}, 11, 115--149. 


 \r A.R.Barron (1984) Predicted Squared Error: A Criterion for 
 Automatic Model Selection. in  Farlow (1984). 


 \r D.Basu (1988). Statistical Information and Likelihood.  
 Edited by J.K.Ghosh. {\it Lect. Notes in Statistics}, 45.  

 \r D.Basu, J.K.Ghosh (1988). Statistical Information and Likelihood.  
  %Edited by J.K.Ghosh (ed.)  
  {\it Lecture Notes in Statistics,} 45.  

 \r D.Basu, C.A.B.Pereira (1982). On the Bayesian Analysis of
 Categorical Data: The Problem of Nonresponse. 
 {\it JSPI} 6, 345-62. 

 \r D.Basu, C.A.B.Pereira (1983). A Note on Blackwell Sufficiency and a
 Shibinsky Characterization of Distributions. 
 {\it Sankhya A}, 45,1, 99-104.


 \r M.S.Bazaraa, H.D.Sherali, C.M.Shetty (1993). {\it Nonlinear 
 Programming: Theory and Algorithms.} NY: Wiley. 

 %\r R.A.Becker, J.M.Chambers (1984).
 %{\it S An Interactive Environment for Data Analysis and Graphics}.
 %Pacific Grove: Wadsworth Statistics/Probability series.

 \r J.L.Bell (1998). {\it A Primer of Infinitesimal Analysis.} 
    Cambridge Univ. Press. 

 \r J.L.Bell (2005). {\it The Continuous and the Infinitesimal 
    in Mathematics and Philosophy.} Milano: Polimetrica.  

 \r A.H. Benade (1992). {\it Horns, Strings, and Harmony.} 
   Mineola: Dover.  

 \r C.H.Bennett (1976). Efficient Estimation of Free Energy 
 Differences from Monte Carlo Data. 
 {\it Journal of Computational Physics} 22, 245-268. 


 \r J.Beran (1994). {\it Statistics of Long-Memory Processes.} 
 London: Chapman and Hall. 

 \r H.C.Berg (1993). {\it Random Walks in Biology.} 
 Princeton Univ. Press.  

 \r C.A.Bernaards, R.I.Jennrich (2005). Gradient Projection
 Algorithms and Software for Arbitrary Rotation Criteria in Factor
 Analysis. {\it Educational and Psychological Measurement}, 65 (5), 676-696. 

 \r L.von Bertalanffy (1969). General System Theory. 
    NY: George Braziller. 

 \r D.P.Bertzekas, J.N.Tsitsiklis (1989). 
 {\it Parallel and Distributed Computation, Numerical Methods.} 
 Englewood Cliffs: Prentice Hall.  

 \r P.J.Bickel, K.A.Doksum (2001).  
 {\it Mathematical Statistics, 2nd ed.} USA: Prentice Hall. 

 \r C.Biernacki G.Govaert (1998). Choosing Models in Model-based 
 Clustering and Discriminant Analysis. 
 Technical Report INRIA-3509-1998. 

 \r K.Binder (1986).
 {\it Monte Carlo methods in Statistical Physics}. 
 Topics in current Physics 7. Berlin: Springer.

 \r K.Binder, D.W.Heermann (2002). {\it Monte Carlo Simulation in 
 Statistical Physics, 4th ed.} NY: Springer.   

 \r E.G.Birgin, R.Castillo, J.M.Martinez (2004). Numerical comparison of 
 Augmented Lagrangian algorithms for nonconvex problems. to appear in 
 {\it Computational Optimization and Applications.} 

 \r A.Birnbaum (1962). On the Foundations of Statistical Inference. 
 {\it J. Amer. Statist. Assoc.} 57, 269--326.  

 \r A.Birnbaum (1972). More on Concepts of Statistical Evidence. 
 {\it J. Amer. Statist. Assoc.} 67, 858--861. 
 
 \r Z.W.Birnbaum, J.D.Esary, S.C.Saunders (1961). 
 Multicomponent Systems and Structures, and their Reliability. 
 {Technometrics,} 3, 55-77. 

 \r B.Bj\"{o}rkholm, M.Sj\"{o}lund,, P.G.Falk, O.G.Berg, L.Engstrand, 
 D.I.Andersson (2001).  
 Mutation Frequency and Biological Cost of Antibiotic Resistance in 
 Helicobacter Pylori.  {\it PNAS}, 98,4, 14607-14612. 

 \r D.Blackwell, M.A.Girshick (1954). {\it Theory of Games and Statistical 
 Decisions}. NY: Dover reprint (1976). 

 \r J.R.S.Blair, B.Peyton (1993). An Introduction to Chordal Graphs 
    and Clique Trees. In George et al. (1993). 

 \r C.R.Blyth (1972). On Simpson's Paradox and the Sure-Thing Principle. 
 {\it Journal of the American Statistical Association}, 67, p. 364. 

 \r R.D.Bock, R.E.Bargnann (1966). Analysis of Covariance 
 Structure. {\it Psycometrica}, 31, 507--534. 

 \r N.Bohr (1935). {\it Space-Time Continuity and Atomic Physics.}  
  H.H.Wills Memorial Lecture, Univ. of Bristol, Oct. 5, 1931. 
  In Niels Bohr Collected Works, 6, 363-370. 
  Complementarity, p.369-370. 

 \r N.H.D.Bohr (1987a).  
    {\it The Philosophical Writings of Niels Bohr.} 
    V.I- Atomic Theory and the Description of Nature. 
    Woodbridge, Connecticut: Ox Bow Press. 

 \r N.H.D.Bohr (1987b). 
    {\it The Philosophical Writings of Niels Bohr.} 
    V.II- Essays 1932-1957 on Atomic Physics and Human Knowledge. 
    Woodbridge, Connecticut: Ox Bow Press. 

 \r N.H.D.Bohr (1987c). 
    {\it The Philosophical Writings of Niels Bohr.} 
    V.III- Essays 1958-1962 on Atomic Physics and Human Knowledge . 
    Woodbridge, Connecticut: Ox Bow Press. 


 \r N.H.D.Bohr (1999), J.Faye, H.J.Folse, eds. 
    {\it The Philosophical Writings of Niels Bohr.} 
    V.IV- Causality and Complementarity: Supplementary Papers. 
    Woodbridge, Connecticut: Ox Bow Press. 


 \r N.H.D.Bohr (1985), J.Kalckar ed. {\it Collected Works.}  
    V.6- Foundations of Quantum Physics I, (1926-1932). 
    Elsevier Scientific. 

 \r N.H.D.Bohr (1996), J.Kalckar ed. {\it Collected Works.}  
    V.7- Foundations of Quantum Physics II, (1933-1958).  
    Elsevier Scientific. 

 \r N.H.D.Bohr (2000), D.Favrholdt ed. {\it Collected Works.}  
    V.10- Complementarity beyond Physics, (1928-1962).  
    Elsevier Scientific. 
 
 \r N.H.D.Bohr (2007). Questions Answered by Niels Bohr (1885-1962).  
  {\it Physikalisch-Technische Bundesanstalt.}   
 {\tt http://www.ptb.de/en/publikationen/blickpunkt/interviews/bohr.html.}  


 \r J.A.Bonaccini (2000). 
 {\it Kant e o Problema da Coisa Em Si No Idealismo Alem\~{a}o.} 
 SP: Relume Dumar\'{a}.  

 \r W.Boothby (2002). 
 {\it An Introduction to Differential Manifolds and 
   Riemannian Geometry.} NY: Academic Press.

 \r J.Bopry (2002). Semiotics, Epistemology, and Inquiry. 
 {\it Teaching \& Learning,} 17, 1, 5--18. 

 \r K.C. Border (1989). {\it Fixed Point Theorems with Applications 
   to Economics and Game Theory.}  Cambridge University Press. 
 

 \r W.Borges, J.M.Stern (2005). 
 On the Truth Value of Complex Hypothesis.  
 {\it CIMCA-2005 - International Conference on Computational 
 Intelligence for Modelling Control and Automation.} USA: IEEE.  

 \r W.Borges, J.M.Stern (2006). Evidence and Compositionality.   
    p.307-315 in J.Lawry et al.,  
    {\it Soft Methods for Integrated Uncertainty Modelling.}      
    NY: Springer.  

 \r G.E.P.Box, W.G.Hunter, J.S.Hunter (1978).
  {\it Statistics for Experimenters. An Introduction to Design, Data
  Analysis and Model Building.} NY: Wiley.

 \r G.E.Box, G.M.Jenkins (1976). {\it Time Series Analysis, 
  Forcasting and Control.} Oakland: Holden-Day. 

 \r G.E.P.Box and G.C.Tiao (1973). 
 {\it Bayesian Inference in Statistical Analysis.} 
 London: Addison-Wesley. 

 \r   P.J.Bowler (1974). Darwin's Concept of Variation. {\it Journal 
  of the History of Medicine and Allied Sciences}, 29, 196-212.  

 \r  R.Boyd, P.Gasper, J.D.Trout, (1991).  
 {\it The Philosophy of Science.} MIT Press.  

 \r L.M.Bregman  (1967). The Relaxation Method for Finding the 
 Common Point Convex Sets and its Application to the Solution of 
 Problems in Convex Programming. {\it USSR Computational Mathematics 
 and Mathematical Physics,} 7, 200-217.   

 \r L.Breiman, J.H.Friedman, C.J.Stone (1993). 
 {\it Classification and Regression Trees.} Chapman and Hall. 

 \r R.Brent, J.Bruck (2006). Can Computers Help to Explain Biology?  
  {\it Nature}, 440/23, 416--417.  

 \r S.Brier (1995) Cyber-Semiotics: 
 On autopoiesis, code-duality and sign games in bio-semiotics. 
 Cybernetics and Human Knowing, 3, 1, 3--14.   

 \r S.Brier (2001). Cybersemiotics and Umweltlehre. {\it Semiotica},  
 Special issue on Jakob von Uexk\"{u}ll's Umweltsbiologie, 
 134 (1/4), 779-814.

 \r S.Brier (2005). The Construction of Information and Communication: 
 A Cyber-Semiotic Re-Entry into Heinz von Foerster's Metaphysical 
 Construction of Second Order Cybernetics. 
 {\it Semiotica,} 154, 355--399.   

 \r P.J.Brockwell, R.A.Davis (1991). 
 {\it Time Series: Theory and Methods.}  NY: Springer. 

 \r L.de Broglie (1946). {\it Matter and Light.} NY:Dover. 

 \r M.W.Browne (1974). Gradient Methods for Analytical Rotation. 
 {\it British J.of Mathematical and Statistical Psychology}, 27, 115-121. 

 \r M.W.Browne (2001). An Overview of Analytic Rotation in Exploratory
 Factor Analysis. {\it Multivariate Behavioral Research}, 36, 111-150.

 \r P.Brunet (1938). {\it \'{E}tude Historique sur le Principe de la 
 Moindre Action.} Paris: Hermann.   

 \r S.G.Brush (1961). Functional Integrals in Statistical Physics. 
 {\it Review of Modern Physics}, 33, 79-79. 

 \r S.Brush (1968). A History of Random Processes: Brownian Movement from
 Brown to Perrin. {\it Arch. Hist. Exact Sci.} 5, 1-36. 

 \r L.W.Buss (2007). {\it The Evolution of Individuality.} 
 Princeton University Press.  

 \r A.M.S.Bueno, C.A.B.Pereira, M.N.Rabelo-Gay, J.M.Stern (2002). 
 Environmental Genotoxicity Evaluation: Bayesian Approach for a 
 Mixture Statistical Model. {\it Stochastic Environmental Research 
 and Risk Assessment,} 16, 267-278.  

 \r J.R.Bunch, D.J.Rose (1976). {\it Sparse Matrix Computations}.
    NY: Academic Press.   

 \r A.Bunde, S.Havlin (1994). {\it Fractals in Science.} 
  NY: Springer.  
 
 \r E.Butkov (1968). {\it Mathematical Physics.} Addison-Wesley. 

 \r F.W.Byron Jr., R.W.Fuller (1969). 
  Reading, MA: Addison-Wesley.    


 \r T.Y.Cao (2003). Structural Realism and the Interpretation of 
  Quantum Field Theory. {\it Synthese}, 136, 1, 3-24. 

  \r T.Y.Cao (2003). Ontological Relativity and Fundamentality - 
  Is Quantum Field Theory the Fundamental Theory?  
  {\it Synthese}, 136, 1, 25-30.  

  \r T.Y.Cao (2003). Can We Dissolve Physical Entities into 
  Mathematical Structures? {\it Synthese}, 136, 1, 57-71. 

  \r T.Y.Cao (2003). What is Ontological Synthesis? A Reply to Simon 
  Saunders. {\it Synthese}, 136, 1, 107-126. 

  \r T.Y.Cao (2004). Ontology and Scientific Explanation. 
  In Conwell (2004).  

  \r M.Carmeli, S.M.Malin (1976). {\it Representation of the Rotation 
  and Lorentz Groups}. Basel: Marcel Dekker.  

 \r M.P.do Carmo (1976). 
  {\it Differential Geometry of Curves and Surfaces.} 
  NY: Prentice Hall.   

 \r  H.Caygill (1995). %A 
 {\it A Kant Dictionary.} Oxford: Blackwell. 

 \r G.Celeux, G.Govaert (1995). Gaussian Parsimonious Clustering 
 Models. {\it Pattern Recog.} 28, 781-793.


 \r G.Celeux, D.Chauveau, J.Diebolt (1996). 
 On Stochastic Versions of the EM Algorithm. 
 An Experimental Study in the mixture Case. 
 {\it Journal of Statistical Computation and Simulation,} 55, 287--314. 

 \r Y.Censor, S.Zenios (1994). {\it Introduction to Methods of 
 Parallel Optimization.} IMPA, Rio de janeiro. 

 \r Y.Censor, S.A.Zenios (1997). {\it Parallel Optimization: 
  Theory, Algorithms, and Applications.} NY: Oxford. 

 \r C.Cercignani (1998). {\it Ludwig Boltzmann, 
 The Man who Trusted Atoms.}  Oxford Univ. 

  \r M.Ceruti (1989). {\it La Danza che Crea.} Milano: Feltrinelli.  

 \r G.Chaitin (2004). On the Intelligibility of the Universe and the
 Notions of Simplicity, Complexity and Irreducibility.   
 pp. 517-534 in {\it Grenzen und Grenzberschreitungen, XIX.} 
 %Deutscher Kongress f\"{u}r
 %Philosophie, Bonn, 23.-27. September 2002, Vortrge und Kolloquien,
 %Herausgegeben von Wolfram Hogrebe in Verbindung mit Joachim Bromand,
 Berlin: Akademie Verlag.    

 \r L.Chang (2005). Generalized Constraint-Based Inference. 
 M.S.Thesis, Univ.of British Columbia. 

 \r V.Cherkaasky, F.Mulier (1998). {\it Learning from Data.} 
 Wiley, N.Y.  

 \r U.Cherubini, E.Luciano, W.Vecchiato (2004). 
 {\it Copula Methods in Finance.} NY: Wiley. 

 \r J.Y.Ching, A.K.C.Wong, K.C.C.Chan. ``Class-Dependent
 Discretization for Inductive Learning from Continuous and Mixed-Mode
 Data.'' {\it IEEE Transactions on Pattern Analysis and Machine
 Intelligence}, 17 n.7,  pp.641-651, 1995. 

 \r  J.Christis (2001). Luhmann's Theory of Knowledge: 
 Beyond Realism and Constructivism?  {\it Soziale Systeme,} 
 7, 328--349. 

 \r G.C.Chow (1983). {\it Econometrics.} Singapore: McGraw-Hill. 

 \r A.Cichockt, R.Zdunek, S.I.Amari (0000). 
    New Algorithms for Non-Negative Matrix Factorization in 
    Applications to Bild Source Separaton. 

 \r A.Cichockt, S.I.Amari, R.Zdunek, R.Kompass, G.Hori, 
    Z.He (0000). Extended SMART Algorithms for Non-Negative 
    Matrix Factorization. 
 
 \r A.Cichockt, R.Zdunek, S.I.Amari (0000). 
    Csisz\'{a}r's Divergences for Non-Negative Matrix Factorization: 
    Family of New Algorithms. 

 \r G.W.Cobb (1998). {\it Introduction to Design and Analysis of 
    Experiments.} NY: Springer. 

 \r D.W.Cohen (1989). {\it An Introduction to Hilbert Space and 
  Quantum Logic.} NY: Springer. 

 \r R.W.Colby (1988). {\it The Encyclopedia of Technical Market Indicators.} 
  Homewood: Dow Jones - Irwin. 

 \r N.E.Collins, R.W. Eglese, B.L. Golden (1988).
 {\it Simulated Annealing, An Annotated Bibliography}.
 In Johnson (1988).

 \r M.L.L.Conde (1998). 
 {\it Wittgenstein: Linguagem e Mundo.}  
 SP: Annablume. 

 \r P.C.Consul (1989). {\it Generalized Poisson Distributions.} 
  Basel: Marcel Dekker. 

 \r W.J.Cook, W.H.Cunningham, W.R.Pulleyblank, A.Schrijver (1997).  
  {\it Combinatorial Optimization.} Wiley. 

 \r Cornwell (2004). {\it  Explanations: Styles of Explanation in 
    Science.}  

 \r N.C.A.Costa (1963). Calculs Propositionnels pour les
  Systemes Formales Incosistants.
  {\it Compte Rendu Acad. des Scienes,} 257, 3790--3792.


 \r N.C.A.da Costa, D. Krause (2004). 
    Complementarity and Paraconsistency. 
    In Rahman et al. (2004, 1, 557-568). 


 \r N.C.A.Costa, V.S.Subrahmanian (1989).
  Paraconsistent Logics as a Formalism for Reasoning about
  Inconsistent Knowledge Bases.
  {\it Artificial Inteligence in Medicine}, 1, 167--174.

 \r N.C.A.Costa, C.A.Vago, V.S.Subrahmanian (1991).
  Paraconsistent Logics Ptt.
  {\it Zeitschrift f\"{u}r Mathematische Logik und Grundlagen
  der Mathematik}, 37, 139-148.

 \r N.C.A.Costa, J.M.Abe, V.S.Subrahmanian (1991).
  Remarks on Annotated Logic.
  {\it Zeitschrift f\"{u}r Mathematische Logik und Grundlagen 
  der Mathematik}, 37, 561--570.

 \r N.C.A.Costa, J.M.Abe, A.C.Murolo, J.I.da Silva, C.F.S.Casemiro
  (1999). L\'{o}gica Paraconsistente Aplicada. S\~{a}o Paulo: Atlas.

 \r F.G.Cozman (2000). Generalizing Variable Elimination in Bayesian 
  Networks. Proceedings of the Workshop in Probabilistic Reasoning in 
  Artificial Inteligence. Atibaia.  

 \r J.F.Crow (1988). The Importance of Recombination. ch4, p.57-75 in 
  Michod and Levin (1988). 
 
 \r I.Csiszar (1974). Information Measures. 
 {\it 7th Prage Conf.of Information Theory,} 2, 73-86. 

 \r T.van Cutsem. ``Decision Trees for Detecting Emergency Voltage
 Conditions.'' {\it Proc. Second International Workshop on Bulk Power 
 System Voltage Phenomena}, pp.229-240, McHenry, USA, 1991. 

 \r A. Damodaran (2003). {\it Investment Philosophies: Successful
  Investment Philosophies and the Greatest Investors Who Made Them Work.} 
  Wiley. 

 \r  A.Y.Darwiche, M.L.Ginsberg (1992). 
  A Symbolic Generalization of Probability Theory. 
  {AAAI-92.}  
  %{10-th National Conference on Artificial Intelligence.}
  %{10-th Conference of the American Association for Artificial Intelligence.}   
  {10-th Conf. American Association for Artificial Intelligence.}   

 \r A.Y.Darwiche (1993). {\it A Symbolic Generalization 
 of Probability Theory.} Ph.D. Thesis, Stanford Univ.  


 \r C.Darwin (1860). Letter to Asa Gray, dated 3 April 1860. 
 in F.Darwin ed. (1911). The Life and Letters of Charles Darwin, 
 London: John Murray. 

 \r F.N.David (1969). {\it Games, Gods and Gambling. A History of 
 Probability and Statistical Ideas.} London: Charles Griffin. 

 \r L.Davis ed. (1987). Genetic Algorithms and Simulated Annealing. 
 Pittman, 1987.
 
 \r L.Davis, M.Steenstrup (1987). Genetic Algorithms and Simulated 
 Annealing: An Overview. p.1-11 in Davis (1987). 

 \r M.Davis (1977). {\it Applied Nonstandard Analysis.} 
    NY: Dover. 

 \r M.H.DeGroot (1970). {\it Optimal Statistical Decisions}.
  NY: McGraw-Hill.

 \r T. Dehue (1997). Deception, Efficiency, and Random Groups: 
  Psychology and the Gradual Origination of the Random Group Design.  
  {\it Isis}, 88, 4, p.653-673 

 \r A.Deitmar (2005). {\it A First Course in Harmonic Analysis}, 
    2nd ed. NY: Springer.  

 \r B.P.Demidovich, I.A.Maron (1976). {\it Computational Mathematics.} 
  Moskow: MIR. 

 \r A.P.Dempster, N.M.Laird, D.B.Rubin (1977). 
 Maximum Likelihood from Incomplete Data via the EM Algorithm. 
 {\it J. of the Royal Statistical Society B.} 39, 1-38.   


 \r D.G.T.Denison, C.C.Holmes, B.K.Mallick, A.F.M.Smith (2002). 
  {\it Bayesian Methods for Nonlinear Classification and Regression.} 
  John Wiley.  

 \r I.S.Dhillon, S.Sra (0000). Generalized Nonnegative Matrix 
    Approximations with Bregman Divergences. 

 \r P.Diaconis (1978). Statistical Problems in ESP Research. 
    {\it Science}, 201, 131-136. 

 \r P.Diaconis, D.Freeman (1987). A Dozen de Finetti Style Results 
 in Search of a Theory. {\it Ann. Inst. Poincar\'{e} Probab. Stat.}, 
 23, 397--423.  

 \r P.Diaconis (1988). 
 {\it Group Representation in Probability and Statistics.}  
 Hayward: IMA. %Institute of Mathematical Statistics.  

 \r J.M.Dickey (1983). Multiple Hypergeometric Functions: Probabilistic
  Interpretations and Statistical Uses. {\it JASA}, 78, 628-37.

 \r J.M.Dickey, T.J.Jiang, J.B.Kadane (1987). Bayesian Methods for
   Categorical Data. {\it JASA} 82, 773-81.

 \r P.DiMaggio, W.W.Powell (1991).  
 {\it New Institutionalism in Organizational Analysis.} 
 Chicago Univ. 

 \r B.Dodson (1994). {\it Weibull Analysis.} Milwaukee: ASQC Quality Press.

 \r  M.G.Doncel, A.Hermann, L.Michel, A.Pais (1987). 
 {\it Symmetries in Physics (1600-1980).} 
 Seminari d'Hist\`{o}ria des les Ci\`{e}nces. 
 Universitat Aut\`{o}noma de Barcelona. 

 \r I.M.L. D'Otaviano, M.E.Q.Gonzales (2000). 
 {\it Auto-Organiza\c{c}\~{a}o, Estudos Interdisciplinares.} 
 Campinas, Brazil: CLE-UNICAMP.  

 \r  L.E.Dubins L.J.Savage (1965). 
 {\it How to Gamble If You Must. 
 Inequalities for Stochastic Processes.}  
 NY: McGraw-Hill.   

 \r J.Dugundji (1966). {\it Topology.} Boston: Allyn and Bacon. 

 \r I.S.Duff (1986).
 {\it Direct methods for sparse matrices}.
 Oxford: Clarendon Press.
 
 \r R.Dugas (1988). {\it A History of Mechanics.} Dover.  

 \r J.S.Dugdale (1996). 
 {\it Entropy and Its Physical Meaning.} %London: 
 Taylor \& Francis. 

  \r L.E.Durbins and L.J.Savage (1976). {\it How to Gamble if You Must:  
    Inequalities for Stochastic Processes.} NY: Dover. 

 \r M.L.Eaton (1989). 
 {\it Group Invariance Applications in Statistics.} 
 Hayward: IMA. %Institute of Mathematical Statistics.  
 %and American Statistical Association.  

  \r   G.T.Eble (1999). On the Dual Nature of Chance in Evolutionary 
  Biology and Paleobiology. {\it Paleobilogy}, 25, 75-87. 

 \r J.S.Efran, M.D.Lukens, R,J,Lukens (1990).   
 {\it Language, Structure and Change: Frameworks of Meaning in 
 Psychotherapy.} W.W.Norton. 

 \r I.Eibel-Eibesfeldt (1970). {\it Ethology, The Biology of Behavior.} 
     NY: Holt, Rinehart and Winston. 

 \r C.Eisele edt. (1976). 
    {\it The New Elements of Mathematics of Charles S. Peirce.} 
    The Hague: Mouton.     


 \r A.Einstein (1905a). 
 \"{U}ber einen die Erzeugung und Verwandlung des Lichtes betreffenden
 heuristischen Gesichtspunkt. 
 (On a heuristic viewpoint concerning the production and
 transformation of light).  
 {\it Annalen der Physik}, 17, 132-148. 

 \r A.Einstein (1905b). 
 \"{U}ber die von der molekularkinetischen Theorie der W\"{a}rme
 geforderte Bewegung von in ruhenden Fl\"{u}ssigkeiten suspendierten
 Teilchen. 
 (On the motion of small particles suspended in liquids at rest
 required by the molecular-kinetic theory of heat). 
 {\it Annalen der Physik}, 17, 549-560. 

 \r A.Einstein (1905c). 
 Zur Elektrodynamik bewegter K\"{o}rper. 
 (On the Electrodynamics of Moving Bodies). 
 {\it Annalen der Physik}, 17, 891-921. 

 \r A.Einstein (1905d). 
 Ist die T\"{a}rgheit eines Kr\"{o}pers von seinem Energiegehalt 
 abh\"{a}ngig?
 (Does the Inertia of a Body Depend Upon Its Energy Content?). 
 {\it Annalen der Physik}, 18, 639-641. 

 \r A.Einstein (1905, 1956).  
 {\it Investigations on the Theory of the Brownian Movement.} 
 Dover. 

 \r A.Einstein (1950). On the Generalized Theory of Gravitation. 
  {Scientific American,} 182, 4, 13-17. 
  Reprinted in Einstein (1950, 341-355). 

 \r A.Einstein (1954). {\it Ideas and Opinions}. Wings Books.  
  % Mein Weltbild. 

 \r A.Einstein (1991). {\it Autobiographical Notes: A Centennial 
    Edition.} Open Court Publishing Company. 


 \r P.Embrechts (2002). Selfsimilar Processes
 Princeton University Press. 

 \r C.Emmeche, J.Hoffmeyer (1991). From Language to Nature:  
    The Semiotic Metaphor in Biology. {\it Semiotica,}  84, 1/2, 1-42.   

 \r Harald A Enge, M.R.Wehr, J.A.Richards (1972). 
  {\it Introduction to Atomic Physics.}  NY: Addison-Wesley. 

 \r T.Elfving (1980). On Some Methods for Entropy maximization and 
 Matrix Scaling. {\it Linear algebra and its applications,} 34, 321-339. 

 \r A.G. Exp\'{o}sito, L.G. Franquelo (1987).
 A New Contribution to the Cluster Problem. 
 {\it IEEE Transactions on Circuits and Systems}, 34, 546-552.


 \r M.Evans (1997). Bayesian Inference Procedures Derived via
 the Concept of Relative Surprise.
 {\it Communications in Statistics}, 26, 1125--1143. 

 \r M.Evans, T.Swartz  (2000).  {\it Approximating Integrals via Monte
 Carlo and Deterministic Methods.} Oxford University Press.

 \r B.S.Everitt (1984). {\it Latent Variable Models.} 
  London: Chapman and Hall. 

 \r S.C.Fang, J.R.Rajasekera, H.S.J.Tsao (1997). {\it Entropy Optimization 
 and Mathematical Programming.} Kluwer, Dordrecht. 

 \r S.J. Farlow (1984) {\it Self-Organizing Methods in Modeling: 
 GMDH-type Algorithms.} Marcel Dekker, Basel.  
  
 \r J.Feder (1988). {\it Fractals.} NY: Plenum.    

 \r W.Feller (1957). {\it An Introduction to Probability Theory and Its
 Applications} (2nd ed.), V.I. New York: Wiley.

 \r W.Feller (1966). {\it An Introduction to Probability Theory and Its
 Applications} (2nd ed.), V.II. New York, Wiley.

 %\r W.Feller (1971). {\it An Introduction to Probability Theory and 
 %Its Applications} V.2. NY: Wiley. 

 \r  T.S.Ferguson (1996). {\it A Course in Large Sample Theory.} 
 NY: Chapman \& Hall.

 \r J.Ferreira (2006). {\it Semiotic Explorations in Computer Interface 
    Design.} Wellington: Victoria University.    

 \r Feyerabend,P. (1993). {\it Against Method.} Verso Books.  

 \r C.M. Fiduccia, R.M. Mattheyses (1982).
 A Linear Time Heuristic for Improving Network Partitions.
 {\it IEEE Design Automation Conferences}, 19, 175-181.

 \r E.C.Fieller (1954). Some Problems in Interval Estimation. 
 {\it Journal of the Royal Statistical Society B,} 16, 175-185.   

 \r B.de Finetti (1947). La pr\'{e}vision: Des lois logiques, ses sourses
 subjectives. Annalles de l'Institut Henri Poincar\'{e} 7,1-68. English
 translation:  Foresight: Its logical laws, its subjective sources, in
 Kiburg and Smoker Eds. (1963), Studies in Subjective Probability, 
 p.93-158, New York: Wiley.

 \r B.de Finetti (1972). {\it Probability, Induction and Statistics.} 
 NY: Wiley. 

 \r B.de Finetti (1974). {\it Theory of Probability,} 
 V1 and V2. London: Wiley.  

 \r B.de Finetti (1975). {\it Theory of Probability. A Critical 
 Introductory Treatment.} London: John Wiley. 

 \r B.de Finetti (1977). Probabilities of Probabilities: 
  A Real Problem or a Misunderstanding? in 
   A.Aykac and C.Brumat (1977).

 \r B.de Finetti (1980). Probability: Beware of Falsifications. 
    p. 193-224 in: H.Kyburg, H.E.Smokler (1980). {\it Studies in 
    Subjective Probability.} NY: Krieger. 

 \r B.de Finetti (1981). 
 {\it Scritti.} V1: 1926-1930.  Padova: CEDAM

 \r B. de Finetti (1991). 
 {\it Scritti.} V2: 1931-1936. Padova: CEDAM

 \r B.de Finetti (1993). {\it Probabilit\'{a} e Induzione.} 
 Bologna: CLUEB. 

 \r M.A.Finocchiaro (1991). {\it The Galileo Affair: A Documented 
 History.} NY: The Notable Trials Library. 

 \r R.A.Fisher (1935). {\it The Design of Experiments}. 
    8ed.(1966). London: Oliver and Boyd,  
 

 \r R.A.Fisher (1936). The Use of Multiple Measurements in 
 Taxonomic Problems. {\it Annals of Eugenics},7,179--188.   

 \r R.A.Fisher (1926). The arrangement of Field Experiments. 
  {\it Journal of the Ministry of Agriculture}, 33, 503-513.  

 \r H.Flanders (1989). 
 {\it Differential Forms with Applications to the Physical Sciences.} 
 NY: Dover. 

 \r H.Fleming (1979). As Simetrias como Instrumento de Obten\c{c}\~{a}o 
 de Conhecimento. {\it Ci\^{e}ncia e Filosofia,} 1, 99--110. 

 \r  H.von Foerster (2003).
 {\it Understanding Understanding: 
 Essays on Cybernetics and Cognition.}   
 NY: Springer Verlag. 
 The following articles in this anthology are of special interest: \\ 
 (a) On Self-Organizing Systems and their Environments; p.1--19. \\ 
 (b) On Constructing a Reality; p.211--227. \\ 
 (c) Objects: Tokens for Eigen-Behaviors; p.261--271. \\  
 (d) For Niklas Luhmann: How Recursive is Communication? p.305--323. \\  
 (e) Introduction to Natural Magic. p.339--338. 

 \r J.L.Folks (1984). Use of Randomization in Experimental Research. 
  p.17--32 in Hinkelmann (1984). 

 \r H.Folse (1985). {\it The Philosophy of Niels Bohr.} 
    Elsevier. 

 \r C.Fraley, A.E.Raftery (1999). Mclust: Software for Model-Based
  Cluster Analysis. {\it J. Classif.},16,297-306.

 \r J.N.Franklin (1968). {\it Matrix Theory.} 
  Englewood-Cliffs: Prentice-Hall. 

 \r A.P.French (1968). {\it Special Relativity.} 
 NY: Chapman and Hall.  

 \r A.P.French (1974). {\it Vibrations and Waves.} 
    M.I.T. Introductory Physics Series. 

 \r R.Frigg (2005). {\it Models and Representation: Why Structures 
    Are Not Enough.} Tech.Rep. 25/02, Center for Philosophy of Natural 
    and Social Science,  

 \r  S.Fuchs (1996). The new Wars of Truth: 
 Conflicts over science studies as differential modes of observation. 
 {\it Social Science Information,} 307--326. %35, 

 \r M.C.Galavotti (1996). Probabilism and Beyond. 
    {\it Erkenntnis}, 45, 253-265.  

 \r M.V.P.Garcia, C.Humes, J.M.Stern (2002). 
 Generalized Line Criterion for Gauss Seidel Method. 
 {\it Journal of Computational and Applied Mathematics}, 22, 1, 91-97. 

 \r M.R. Garey, D.S. Johnson (1979).
 {\it Computers and Intractability, A Guide to the Theory of NP-Completeness}.
 NY: Freeman and Co. 

 \r R.H.Gaskins (1992). 
 {\it Burdens of Proof in Modern Discourse.} %New Haven: 
 Yale Univ. Press.


 \r  L.A.Gavrilov and N.S.Gavrilova (1991).
 {\it The Biology of Life Span: A Quantitative Approach}. 
 New York: Harwood Academic Publisher.

 \r  L.A.Gavrilov and N.S.Gavrilova (2001). The Reliability Theory of
 Aging and  Longevity. {\it J. Theor. Biol.} 213, 527--545.

 \r R.Karawatzki, J.Leydold, K.P\"{o}tzelberger (2005). Automatic
 Markov Chain  Monte Carlo Procedures for Sampling from Multivariate
 Distributions. Department of Statistics and Mathematics
 Wirtschaftsuniversit\"{a}t Wien Research Report Series. Report 27,
 December 2005.  Software available at
 {\it http://statistik.wu-wien.ac.at/arvag/software.html}. 
 
 %\r A.Gelman, J.B.Carlin, H.S.Stern, D.B.Rubin, (1995).
 % {\it Bayesian Data Analysis.} London: Chapman and Hall. 

 \r A.Gelman, J.B.Carlin, H.S.Stern, D.B.Rubin (2003). 
   {\it Bayesian Data Analysis}, 2nd ed. NY: Chapman and Hall / CRC.    

 \r J.E.Gentle (1998). {\it Random Number Generator and Monte 
  Carlo Methods.} NY: Springer. 


 \r A.M.Geoffrion ed. (1972). {\it Perspectives on Optimization: 
    A Collection of Expository Articles.} NY: Addison-Wesley. 

 \r A.George, J.W.H.Liu (1978). A Quotient Graph Model for Symmetric 
    Factorization. p.154-175 in: I.S.Duff, G.W.Stewart (1978) 
    {\it Spase Matrix Proceedings.} Philadelphia: SIAM. 
 
 \r A.George, J.W.H.Liu, E.Ng (1989). Solution of Sparse Positive 
    Definite Systems on a Hypercube, in: 
    Vorst and van Dooren (1990). 

 \r A.George, J.R.Gilbert, J.W.H.Liu (ed.) (1993). {\it Graph Theory and 
    Sparse Matrix Computation.} NY: Springer. 

 \r A.George, J.W.H.Liu (1981). {\it Computer Solution of Large Sparse 
 Positive-Definite Systems.} NY: Prentice-Hall. 

 \r C.J.Gerhardt (1890). 
 {\it Die philosophischen Schriften von Gottfried Wilhelm Leibniz.}  
 Berlin: Weidmannsche Buchhandlung.  

 \r W.R.Gilks, S.Richardson, D.J.Spiegelhalter (1996). 
 {\it Markov Chain Monte Carlo in Practice.} NY: CRC Press. 
 
 \r M.Ginsberg (1986). Multivalued Logics.
 {\it AAAI-86, 6th National Conference on Artificial Intelligence.}
  243--247.

 \r Z.Ghaharamani, G.E.Hilton (1997). {\it The EM Algorithm for 
  Mixtures of Factor Analyzers.} Tech.Rep. CRG-TR-96-1. 
  Dept. of Computer Science, Univ. of Toronto.  
   

 \r D.E.Goldberg (1989). 
 {\it Genetic Algorithms in Search, Optimization, and Machine Learning}. 
 Reading, MA: Addison-Wesley. 

 \r R.Goldblatt (1998). {\it Lectures on the Hyperreals: 
 An Introduction to Nonstandard Analysis.} NY: Springer.   

 \r L. Goldstein, M. Waterman (1988).
 {\it Neighborhood Size in the Simulated Annealing Algorithm}.
 In Johnson (1988). 

 \r H.H.Goldstine (1980). {\it A History of the Calculus of 
 Variations from the Seventeenth Through the Nineteenth Century}. 
 Studies in the History of Mathematics and the Physical Sciences. 
 NY: Springer. 

 \r M.C.Golumbic (1980). 
 {\it Algorithmic Graph Theory and Perfect Graphs.} NY: Academic Press. 

 \r D.V.Gokhale (1975). Maximum Entropy Characterization of some 
 Distributions. In Patil,G.P., Kotz,G.P., Ord,J.K. {\it Statistical 
 Distributions in Scientific Work.} V-3, 299-304. 

 \r  G.H.Golub, C.F.van Loan (1989). {\it Matrix 
 Computations.} Baltimore: Johns Hopkins.  

 \r I.J.Good (ed.) (1962). {\it The Scientist Speculates. An Anthology 
    of Partly-Baked Ideas.} NY: Basic Books.  
 
 \r  I.J.Good (1983). {\it Good thinking: The foundations of 
 probability and its applications}. 
 Minneapolis: University of Minnesota Press.  
 
 \r I.J.Good (1988). The Interface Between Statistics and Philosophy of 
    Science. {\it Statistical Science}, 3, 4, 386-397. 

 \r I.J.Good, Y.Mittal (1987). The Amalgamation and Geometry of
    Two-by-Two Contingency Tables. {\it Annals of Statistics}, 
    15, p. 695. 

 \r P.C.Gotzsche (2002). Assessment of Bias. In S.Kotz, ed. (2006). 
  {\it The Encyclopedia of Statistics,} 1, 237-240.   

 \r A.L. Goudsmit (1988).  
 Towards a Negative Understanding of Psychotherapy. 
 Ph.D. Thesis, Groningen University.  
 %Section 2.3.3, Objects as warrants for eigenvalues. 

 \r S.Greenland, J.Pearl. J.M.Robins (1999). 
 Confounding and Collapsibility in Causal Inference. 
 {\it Statistical Science}  14, 1, 29-46.

 \r S.Greenland, H.Morgenstern1 (2001). Confounding in Health Research. 
  {\it Annual Review of Public Health}, 22, 189-212.  

 \r J.S.Growney (1998). Planning for Interruptions. 
  {\it Mathematics Magazine}, 55, 4, 213-219. 

 \r  B.Gruber et al. edit. (1980--98). 
 {\it Symmetries in Science, I--X.} NY: Plenum. %Press. 

 \r E.Gunel (1984). A Bayesian Analysis of the Multinomial Model for a
 Dichotomous Response with Non-Respondents. {\it Communications in 
 Statistics - Theory and Methods}, 13, 737-51.

 \r I.Hacking (1988). Telepathy: Origins of Randomization in Experimental 
    Design. {\it Isis}, 79, 3, 427-451.  

 \r O.H\"{a}ggstr\"{o}m (2002). 
 {\it Finite Markov Chains and Algorithmic Applications.} 
 Cambridge Univ.  


 \r P.R.Halmos (1998). {\it Naive Set Theory.} 
    NY: Springer. 

 \r J.H.Halton (1970). A Retrospective and Prospective Survey of 
 the Monte Carlo Method. {\it SIAM Review,} 12, 1, 1-63. 

 \r J.M.Hammersley, D.C.Handscomb (1964). {\it Monte Carlo Methods.} 
 London: Chapman and Hall. 

 \r  J.Hanc, S.Tuleja, M.Hancova (2004). Symmetries and Conservation 
 Laws: Consequenses of Noether's Theorem.  
 {\it American Journal of Physics}, 72, 428--435.   

 \r I.Hargittai (1992). {\it Fivefold Symmetry.} 
 Singapore: World Scientific. 

 \r C.Hartshorne, P.Weiss, A.Burks, edts. (1992).  
  {\it Collected Papers of Charles Sanders Peirce.} 
    Charlottesville: InteLex Corp. 

 \r E.J.Haupt (1998). G.E.M\"{u}ller as a Source of American Psychology. 
 In R.W.Rieber, K.Salzinger, eds. (1998). 
 {\it Psychology: Theoretical-Historical Perspectives.}  
 American Psychological Association. 

 \r D.A.Harville (2000). {\it Matrix Algebra From a Statistician's 
 Perspective}. NY: Springer. 

 \r  L.L.Harlow, S.A.Mulaik, J.H.Steiger (1997). 
 {\it What If There Were No Significance Tests?}  
 London: LEA - Lawrence Erlbaum Associates. 

 \r C.Hartshorne, P.Weiss, A.Burks, edts. (1992).  
    {\it Collected Papers of Charles Sanders Peirce.} 
    Charlottesville: InteLex Corp. 

 \r Harville,D.A. (1997). {\it Matrix Algebra from a 
 Statistician's Perspective}. NY: Springer.  

 \r M.Haw (2002). Colloidal Suspensions, Brownian Motion, Molecular
  Reality: A Short History. {\it J. Phys. Condens. Matter}. 
  14, 7769-7779.  

 \r W.Heisenberg (1958). {\it Physics and Philosophy.} 
 London: Pinguin Classics reprint (2000). 

 \r W.Heitler (1956).  {\it Elementary Wave Mechanics.} 
    Oxford University Press.   
 

 \r E.Hellerman, D.C.Rarick (1971).
 Reinversion with the Preassigned Pivot Procedure. 
 {\it Mathematical Programming}, 1, 195-216.

 \r Helmholtz (1887a). \"{U}ber die physikalische Bedeutung des Princips 
  der keinsten Wirkung. 
 {\it Journal f\"{u}r reine und angewandte Mathematik}, 
 100, 137-166, 213-222.  

 \r Helmholtz (1887b). Zur Geschichte des Princips der kleinsten Action. 
 {\it Sitzungsberichte der K\"{o}niglich Preussichen Akademie der 
 Wissenschaften zu Berlin}, I, 225-236.  

 \r R.J.Hernstein, E.G.Boring (1966). 
 {\it A Source Book in Psychology.} Harvard Univ. 

 \r M.B.Hesse (1966). {\it Models and Analogies in Science.}  
  University of Notre Dame Press. 

 \r M.Heydtmann (2002). The nature of truth: Simpson's Paradox and the 
  Limits of Statistical Data. {\it QJM: An International Journal of 
  Medicine}. 95, 4, 247-249. 

 \r K.Hinkelmann (ed.) (1984). {\it Experimental Design, Statistical 
  Models and Genetic Statistics. Essays in Honor of Oscar Kempthorne.} 
  Basel: Marcel Dekker. 

 \r J.S.U.Hjorth (1984). {\it Computer Intensive Statistical Methods.} 
 Chapman and Hall, London. 

 \r R.R.Hocking (1985). {\it The Analysis of Linear Models.} 
 Monterey: Brooks Cole. 

 \r J.H.Holland (1975). 
 {\it Adaptation in Natural and Artificial Systems.}
 Ann Arbor: University of Michigan Press.

 \r F.H.C.Hotchkiss (1998). A ``Rays-as-Appendages'' Model for the Origin 
  of Pentamerism in Echinoderms.  {\it Paleobiology}, 24,2, 200-214.

 \r R.Houtappel, H.van Dam, E.P.Wigner (1965). The Conceptual Basis 
 and Use of the Geometric Invariance Principles. {\it Reviews of 
 Modern Physics,} 37, 595--632.  

 \r P.O.Hoyer (2004). Non-Negative Matrix Factorizations with Sparseness 
    Constrains. {\it J.of Machine Learning Research}, 5, 1457-1469.  

 \r P.Hoyningen-Huene (1993). 
 {\it Reconstructing Scientific Revolutions. 
  Thomas S. Kuhn's Philosophy of Science.}  
 University of Chicago Press.  

 \r C.Huang, A.Darwiche (1994). Inference in Belief Networks: 
 A Procedural Guide. Int.J.of Approximate Reasoning, 11, 1-58.  

 \r M.D. Huang, F. Roameo, A. Sangiovanni-Vincentelli (1986).
 An Efficient General Cooling Schedule for Simulated Annealing. 
 {\it IEEE International Conference on Computer-Aided Design}, 
 381-384.


 \r R.I.G.Hughes (1992). {\it The Structure and Interpretation of 
  Quantum Mechanics.} Harvard University Press.   

 \r T.P.Hutchinson (1991). {\it The engineering statistician's guide to
 continuous bivariate distributions.} Sydney: Rumsby Scientific Pub. 

 \r H.Iba, T.Sato (1992). Meta-Level Strategy for Genetic Algorithms 
 Based on Structured Representation. p.548-554 in {\it Proc. of the 
 Second Pacific Rim International Conference on Artificial Intelligence.} 


 \r I.A.Ibri (1992). {\it Kosmos Noetos. A Arquitetura Metaf\'{\i}sica 
 de Charles S. Peirce.} S\~{a}o Paulo: Prespectiva. 


 \r B.Ingrao, G.Israel (1990). {\it The Invisible Hand: 
   Economic Equilibrium in the History of Science.} MIT Press.  
 
 \r  T.Z.Irony, M.Lauretto, C.A.B.Pereira, and J.M.Stern (2002). 
 A Weibull Wearout Test: Full Bayesian Approach.
 In: Y.Hayakawa, T.Irony, M.Xie, edit.    
 {Systems and Bayesian Reliability}, 287--300. 
 {\it Quality, Reliability \& Engineering Statistics}, 5, 
 Singapore: World Scientific. 

 \r T.Z.Irony, C.A.B.Pereira (1994). Motivation for the Use of Discrete
 Distributions in Quality Assurance. {\it Test}, 3,2, 181-93.

 \r T.Z.Irony, C.A.B.Pereira (1995), Bayesian Hypothesis Test: Using 
 Surface Integrals To Distribute Prior Information Among The Hypotheses,
 Resenhas, Sao Paulo 2(1): 27-46.

 \r T.Z.Irony, C.A.B.Pereira, R.C.Tiwari (2000). Analysis of Opinion 
 Swing: Comparison of Two Correlated Proportions. {\it The American
 Statistician}, 54, 57-62. 


 \r A.N.Iusem, A.R.De Pierro (1986). Convergence Results for an 
 Accelerated Nonlinear Cimmino Algorithm. {\it Numerische Matematik,}  
 46, 367-378. 

 \r A.N.Iusem (1995). {\it Proximal Point Methods in Optimization.} 
 Rio de Janeiro: IMPA. 

 \r A.J.Izzo (1992). A Functional Analysis Proof of the Existence of Haar 
 Measure on Locally Compact Abelian Groups
 {\it Proceedings of the American Mathematical Society}, 115, 2, 581-583. 

 \r  B.Jaffe (1960). {\it Michelson and the Speed of Light.} 
 NY: Anchor.  

 \r J.Jastrow (1899). The mind's eye. 
 {\it Popular Science Monthly}, 54, 299-312. 
 Reprinted in Jastrow (1900). 
 
 \r J.Jastrow (1900). {\it Fact and Fable in Psychology.} 
  Boston: Houghton Mifflin.

 \r J.Jastrow (1988). A Critique of Psycho-Physic Methods. 
 {\it American Journal of of Psychology}, 1, 271-309.   

 \r R.I.Jennrich (2001). A Simple General Method for Orthogonal Rotation. 
  {\it Psychometrica}, 66, 289-306. 

 \r R.I.Jennrich (2002). A Simple Method for Oblique Rotation. 
 {\it Psychometrika}, 67,1,7-20.  

 \r R.I.Jennrich (2004). Rotation to Simple Loadings using Component
 Loss Functions: The Orthogonal Case. {\it Psychometrika}, 69, 257-274. 

 \r G.Jetschke (1989). On the Convergence of Simulated Annealing. 
 pp. 208-215 in Voigt et al. (1989). 

 \r C.G.Jung (1968). {\it Man and His Symbols.}  Laurel. 

 \r T.J.Jiang, J.B.Kadane,  J.M.Dickey (1992). Computation of Carsons
 Multiple Hipergeometric Function R for Bayesian Applications.  
 {\it Journal of Computational and Graphical Statistics}, 1, 231-51.

 \r Jiang,G., Sarkar,S. (1998). Some Asymptotic Tests for the 
 Equality of Covariance Matrices of Two Dependent Bivariate Normals. 
 {\it Biometrical Journal}, 40, 205--225. 

 \r  Jiang,G., Sarkar,S., Hsuan,F. (1999). A Likelihood Ratio Test  
 and its Modifications for the Homogeneity of the Covariance Matrices of 
 Dependent Multivariate Normals. {\it J. Stat. Plan. Infer.}, 81, 95-111. 

 \r  Jiang,G., Sarkar,S. (2000a). Some Combination Tests for the 
 Equality of Covariance Matrices of Two Dependent Bivariate Normals. 
 Proc. {\it ISAS-2000, Information Systems Analysis and Synthesis.} 

 \r  Jiang,G., Sarkar,S. (2000b). The Likelihood Ratio Test for 
 Homogeneity of the Variances in a Covariance Matrix with Block 
 Compound Symmetry. {\it Commun. Statist. Theory Meth.} 29, 1155-1178.  

 \r D.S.Johnson, C.R.Aragon, L.A.McGeoch, C.Schevon (1989).
 Optimization by Simulated Annealing: An experimental evaluation, part 1.
 {\it Operations Research},  37, 865-892.

 \r M.E.Johnson (1987). Multivariate Statistical Simulation. 
 NY: Wiley. 

 \r M.E. Johnson (ed.) (1988).
 {\it Simulated Annealing \& Optimization}.
 Syracuse: American Science Press. This book is also the volume 8 
 of the {\it American Journal of Mathematical and Management Sciences.} 


 \r  M.C.Jones (1985). Generating Inverse Wishart Matrices. 
 {\it Commun. Statist. Simula. Computa.} 14, 511--514. 
  
 \r  J\"{o}reskog,K.G. (1970). A General Method for Analysis of 
 Covariance Structures. {\it Biometrika}, 57, 239--251.  

 \r J.B.Kadane (1985). Is Victimization Chronic? A Bayesian Analysis of
 Multinomial Missing Data. {\it Journal of Econometrics}, 29, 47-67.

 \r J.Kadane, T.Seidenfeld (1990). Randomization in a Bayesian Perspective. 
    {\it J.of Statistical Planning and Inference}, 25, 329-345. 

 \r J.B.Kadane, R.L.Winkler (1987). De Finetti's Methods of 
 Elicitation. In Viertl (1987).   


 \r I.Kant (1790). Critique of Teleological Judgment. 
 In Kant's Critique of Judgement, Oxford: Clarendon Press, 1980. 
 % Part 11, 4 (65).  

 \r I.Kant. {\it The critique of pure reason; The critique 
             of practical reason; The critique of judgment.} 
 Encyclopaedia Britannica Great books of the Western World, v.42, 1952.   


 \r S.Kaplan, C.Lin (1987). An Improved Condensation Procedure in 
 Discrete Probability Distribution Calculations. 
 {\it Risk Analysis,} 7, 15-19.  

 \r   T.J.Kaptchuk, C.E.Kerr (2004). Commentary: Unbiased Divination, 
  Unbiased Evidence, and the Patulin Cliniacal Trial. 
  {\it International Journal of Epidemiology}, 33, 247-251.  

 \r J.N.Kapur (1989). {\it Maximum Entropy Models in Science and 
 Engineering.}  New Delhi: John Wiley.    

 \r J.N.Kapur, H.K.Kesevan (1992). {\it Entropy Optimization Principles
  with Applications.} Boston: Academic Press. 

 \r T.R.Karlowski, T.C.Chalmers, T.C.Frankel, L.D.Kapikian, 
    T.L.Lewis, J.M.Lynch (1975). Ascorbic acid for the common cold: 
    a prophylactic and therapeutic trial. {\it JAMA}, 231, 1038-1042. 

 \r A.Kaufmann, D.Grouchko, R.Cruon (1977). {\it Mathematical Models 
 for the Study of the Reliability of Systems.} NY: Academic Press. 

 \r M.J.Kearns, U.V.Vazirani (1994). {\it Computational Learning 
 Theory.} Cambridge: MIT Press.  

 \r O.Kempthorne, L.Folks (1971). {\it Probability, Statistics and 
 Data Analysis.} Ames: Iowa State Univ. Press. 

 \r O.Kempthorne (1976). Of what Use are Tests of Significance and 
 Tests of Hypothesis. {\it Comm. Statist.} A5, 763--777. 

 \r O.Kempthorne (1977). Why Randomize? {\it J. of Statistical Planning
    and Inference,} 1, 1-25 

 \r Kempthorne,O. (1980). Foundations of Statistical Thinking and 
 Reasoning. {\it Australian CSIRO-DMS Newsletter.} 68, 1--5; 69, 3--7.  

 \r B.W. Kernighan, S. Lin (1970).
 An Efficient Heuristic Procedure for Partitioning Graphs. 
 {\it The Bell System Technical Journal}, 49, 291-307.

 \r A.I.Khinchin (1953). {\it Mathematical Foundations of Information 
 Theory.} NY: Dover.  

 \r J.F.Kihlstrom (2006). {\it Joseph Jastrow and His Duck - Or Is It 
  a Rabbit?} On line document, University of California at Berkeley. 

 \r D.A.Klein and G.C.Rota (1997). {\it Introduction to Geometric 
 Probability.} Cambridge Univ. Press.  

 \r  G.J.Klir, T.A.Folger (1988). 
 {\it Fuzzy Sets, Uncertainty and Information.} NY: Prentice Hall.    

 \r C.J.W.Kloesel (1993). {\it Writings of Charles S. Peirce. 
    A Chronological Edition}.   

 \r S.Kocherlakota, KKocherlakota (1992). {\it Bivariate Discrete 
 Distributions.} 
 Basel: Marcel Dekker. 

 \r J.Kokott (1998). {\it The Burden of Proof in Comparative and
  International Human Rights Law.}  Hague: Kluwer.


 \r V.B.Kolmanovskii, V.R.Nosov (1986). {\it Stability of Functional 
 Differential Equations.} London: Academic Press. 

  \r A.N.Kolmogorov, S.V.Fomin (1982, Portuguese translation). 
 {\it Elements of the Theory of Functions and Functional Analysis.}    
 Moscow: MIR. 

 \r B.O.Koopman (1940a). Axioms and Algebra of Intuitive 
 Probability. {\it Annals of Mathematics}, 41, 269--292. 

 \r B.O.Koopman (1940b). Bases of Probability. {\it 
 Bulletin of the Ammerican Mathematical Society}, 46, 763--774. 

 \r S.Kotz, N.Balakrishnan, C.B.Read, B.Vidakovic, edts. (2005). 
    {\it Encyclopedia of Statistical Sciences,} 2nd ed. 
    Wiley-Interscience. 
    %On line at www.mrw.interscience.wiley.com/ess. 

 \r J.R.Koza (1989). Hierarchical Genetic Algorithms Operating on 
  Populations of Computer Programs. 
  In Proceedings of the Eleventh International Joint Conference on
  Artificial Intelligence, IJCAI-89, N.S.Sridharan (ed.), 
  vol.1, p.768--774, Morgan Kaufmann. 
 

 \r  K.L.Krasnov, G.I.Makarenko, A.I.Kiseliov (1973, 1984). 
 {\it C\'{a}lculo Variacional}. MIR, Moskow. 

 \r  W.Krohn, G.K\"{u}ppers, H.Nowotny (1990). 
 {\it Selforganization. Portrait of a Scientific Revolution.}  
 Dordrecht: Kluwer. 

 \r  W.Krohn, G. K\"{u}ppers (1990). The Selforganization of  
 Science - Outline of a Theoretical Model.  
 in Krohn (1990), 208--222. 

 \r O.S.Ksenzhek, A.G.Volkov (1998). {\it Plant Energetics.} 
  NY: Academic Press. 

 \r T.S.Kuhn (1977). {\it The Essential Tension: Selected Studies 
    in Scientific Tradition and Change}. University of Chicago Press. 

 \r T.S.Kuhn (1996). {\it The Structure of Scientific Revolutions.} 
 University of Chicago Press. 

 \r C.L.Lanczos (19xx). {\it The Variational Principles of Mechanics.}   
  Noether's Invariant Variational Problems, Appendix II, p.401-405. 
  

 \r D.Landau, K.Binder (2000). {\it A Guide to Monte Carlo Simulations 
 in Statistical Physics.} Cambridge University Press.  

 \r L.D.Landau, E. M. Lifchitz (1966). 
 {\it Cours de Physique Th\'{e}orique.} Moscou: MIR. 

 \r I.Lakatos (1978a). {\it The Methodology of Scientific Research.} 
 Cambridge Univ. Press. 

 \r I.Lakatos (1978b). {\it Mathematics, Science and Epistemology.} 
 Canbridge Univ. Press. 

 \r G.Lakoff, M.Johnson (2003). {\it Metaphors We Live By.} 
 University of Chicago Press. 

 \r P.J.M. van Laarhoven, E.H.L. Aarts (1987).
 {\it Simulated Annealing: Theory and Applications}.
 Dordrecht: Reidel Publishing Co. 

 \r L.S.Lasdon (1970). {\it Optimization Theory for Large Systems.} 
    NY: MacMillan. 

 \r M.Lauretto, F.Nakano, C.A.B.Pereira, J.M.Stern (1995). 
    Editora Abril / DINAP Sales Forcast Consulting Project. 
    Unpublished report.  

 \r   M.Lauretto, C.A.B.Pereira, J.M.Stern, S.Zacks (2003).
 Full Bayesian Significance Test Applied to Multivariate Normal 
 Structure Models.  
 %Comparing Parameters of Two Bivariate Normal Distributions Using the
 %Invariant Full Bayesian Significance Test.
 {\it Brazilian Journal of Probability and Statistics,} 17, 147-168. 

 \r M.Lauretto, F.Nakano, C.O.Ribeiro, J.M.Stern (1998). 
 REAL: Real Attribute Learning Algorithm. 
 ISAS-98 Proceedings, 2, 315-321.   

 \r M.Lauretto, J.M.Stern (2005). FBST for Mixture Model Selection. 
 MaxEnt 2005, 24th International Workshop on Bayesian Inference 
 and Maximum Entropy Methods in Science and Engineering. 
 {\it American Institute of Physics Conference Proceedings}, 
 803, 121--128.  

  \r M.Lauretto, S.R. de Faria Jr., B.B.Pereira, 
   C.A.B.Perreira, J.M.Stern (2007).  
  The Problem of Separate Hypotheses via Mixture Models. To appear, 
  {\it American Institute of Physics Conference Proceedings}.  


 \r S.L.Lauritzen (2006). {\it Fundamentals of Graphical Models.} 
    Saint Flour Summer-school.   

 \r J.W.Leech (1963). {\it Classical Mechanics.} London: Methuen. 

 \r Lehmann,E.L. (1959). {\it Testing Statistical Hypothesis.} 
 NY: Wiley.  

 \r D.S.Lemons (2002).  {\it An Introduction to Stochastic Processes in 
  Physics.} Baltimore: John Hopkins Univ. Press. 

 \r    T.Lenoir (1982). {\it The Strategy of Life. Teleology and Mechanics 
 in Nineteenth-Century German Biology.} Univ.of Chicago Press. 

 \r  I.Levi (1974). {\it Gambling with Truth: 
 An Essay on Induction and the Aims of Science.}  
 MIT Press. 

 \r  D.V.Lindley (1957). A Statistical Paradox. 
 {\it Biometrika} 44, 187--192.  

 \r D.V.Lindley (1991). {\it Making Decisions.} NY: John Wiley.  

 \r D.V.Lindley, M.R.Novick (1981). The Role of Exchangeability in 
    Inference. {it The Annals of Statistics}, 9, 1, 45-58. 

 \r R.J.A.Little, D.B.Rubin (1987). {\it Statistical Analysis with 
 Missing Data.} New York: Wiley.

 \r J.L.Liu (2001). {\it Monte Carlo Strategies in Scientific Computing.} 
 NY: Springer. 

 \r D.Loemker (1969). 
  {\it G.W.Leibniz Philosophical Papers and Letters.}  
  Reidel.

 \r  H.A.Lorentz, A.Einstein, H.Minkowski and H.Weyl (1952). 
 {\it The Principle of Relativity: A Collection of Original Memoirs 
 on the Special and General Theory of Relativity.} 
 NY: Dover.

 \r R.H.Loschi, S.Wechsler (2002). {\it Coherence, Bayes's 
 Theorem and Posterior Distributions}, Brazilian Journal of 
 Probability and Statistics, 16, 169--185. 

 \r D.G.Luenberger (1984). {\it Linear and Nonlinear Programming.} 
  Reading: Addison-Wesley. 

 \r  N.Luhmann (1989). 
 {\it Ecological Communication.}  Chicago Univ. Press. 

 \r   N.Luhmann (1990a). {\it The Cognitive Program of 
 Constructivism and a Reality that Remains Unknown.} 
 in Krohn (1990), 64--86. 

 \r  N.Luhmann (1990b). {\it Essays on Self-Reference.}  
 NY: Columbia Univ. Press. 

 \r  N.Luhmann (1995). 
 {\it Social Systems.} Stanford Univ. Press. 

 \r M. Lundy, A. Mees (1986). Convergence of an Annealing Algorithm.
 {\it Mathematical Programming}, 34, 111-124.

 \r I.J.Lustig (1987).
 {\it An Analysis of an Available Set of Linear Programming Test Problems}.
 Tech. Rep. SOL-87-11, Dept. Operations Research, Stanford University.

 \r D.K.C.MacDonald (1962). 
 {\it Noise and Fluctuations: An Introduction.} NY: Wiley.   

 \r H.R.Madala, A.G.Ivakhnenko (1994). {\it Inductive Learning Algorithms
  for Complex Systems Modeling.} Boca Raton: CRC Press.   


 \r H.R.Madala, A.G.Ivakhnenko (1994). 
 {\it Inductive Learning Algorithms for Complex Systems Modeling.}  
 CRC. 

 \r  M.R.Madruga, L.G.Esteves, S.Wechsler (2001).
 On the Bayesianity of Pereira-Stern Tests.
 {\it Test}, 10, 291--299.
 
 \r   M.R.Madruga, C.A.B.Pereira, J.M.Stern (2003).
 Bayesian Evidence Test for Precise Hypotheses.
 {\it Journal of Statistical Planning and Inference,}
  117, 185--198.

 \r  P.Maher, B.Skyrms, E.W.Adams, K.Binmore, J.Butterfield, 
 P.Diaconis, W.L. Harper (1993). {\it Betting on Theories.}  
 Cambridge Univ. Press. 


 \r M.Maimonides (2001). {\it  Mishne Torah: Yad hachazakah.}
 NY: Yeshivath Beth Moshe. 

 \r D.D.Mari, S.Kotz (2001). {\it Correlation and Dependence.} 
    Singapore: World Scientific. 

 \r J.B.Marion (1970). {\it Classical Dynamics of Particles and Systems.} 
 NY:  Academic Press. 

 \r J.B.Marion (1975). {\it Classical Dynamics of Particles and 
    Systems.} NY: Academic Press. 

 \r J.J.Martin (1975). 
 {\it Bayesian decision and probelms and Markov Chains.}  

 \r J.L.Martin (1988). {\it Genearl Relativity. A Guide to its 
  Consequences for Gravity and Cosmology.} 
  Chichester: Ellis Horwood - John Willey.  

 \r J.M.Martinez, J.M. (1999). A Direct Search Method for Nonlinear 
  Programming. {\it ZAMM,} 79, 267-276. 

 \r J.M.Martinez (2000). BOX-QUACAN and the Implementation of 
 Augmented Lagrangian Algorithms for Minimization with Inequality 
 Constraints. {\it Computational and Applied Mathematics.} 19, 31-56.  

  \r  H.R.Maturana, F.J.Varela (1980). 
 {\it Autopoiesis and Cognition. The Realization of the Living.}  
 Dordrecht: Reidel. 

 \r H.R.Maturana (1988). Ontology of Observing. The Biological 
 Foundations of Self Consciousness and the Physical Domain of Existence.  
 pp 18--23 in {\it Conference Workbook: Texts in Cybernetics.} 
 Felton, CA: American Society for Cybernetics.  

 \r H.R.Maturana (1991). Science and Reality in Daily Life: 
    The Ontology of Scientific Explanations. In Steier (1991). 
  
 \r H.R.Maturana, B.Poerksen (2004). Varieties of Objectivity. 
 {\it Cybernetics and Human Knowing.} 11, 4, 63--71. 


 \r P.L.M.de Maupertuis (1965), {\it Oeuvres, I-IV.} 
  Hildesheim: Georg Olms Verlagsbuchhandlung.  
  %FFLCH 194 M452o v.2


 \r G.P. McCormick  (1983).
 {\it Nonlinear Programming: Theory, Algorithms and Applications}.
 Chichester: John Wiley.

 \r D.K.C.MacDonald (1962). {\it Noise and Fluctuations.} NY: Dover. 

 \r  R.P.McDonald (1962). A Note on the Derivation of the General 
 Latent Class Model. {\it Psychometrika} 27, 203--206. 

 \r R.P.McDonald (1974). Testing Pattern Hypotheses for Covariance  
 Matrices. {\it Psychometrika}, 39, 189--201. 

 \r R.P.McDonald (1975). Testing Pattern Hypotheses for Correlation 
 Matrices. {\it Psychometrika}, 40, 253--255. 

 \r R.P.McDonald, H.Swaminathan (1973). A Simple Matrix Calculus 
 with Applications to Multivariate Analysis. 
 {\it General Systems}, 18, 37--54 

  \r A.L.McLean (1998), The Forecasting Voice: A Unified Approach to 
 Teaching Statistics. In {\it Proceedings of the Fifth International 
 Conference on Teaching of Statistics}, (eds L. Pereira-Mendoza, et al.), 
 1193-1199. Singapore: Nanjing University.  


 \r G.McLachlan, D.Peel (2000). {\it Finite Mixture Models.} NY: Wiley. 

 \r W.H.McRea (1954). {\it Relativity Physics}. London: Methuen.  

 \r E.J.McShane. The Calculus of Variations. Ch.7, p.125-130 in: 
 J.W.Brewer, M.K.Smith (19xx). {\it Emmy Noether}.  

 \r   J.G.Mendel (1866). Versuche \"{u}ber Plflanzenhybriden Verhandlungen 
 des naturforschenden Vereines in Br\"{u}nn, Bd. IV f\"{u}r das Jahr, 1865
 Abhandlungen: 3-47. For the English translation, see: Druery, C.T and
 William Bateson (1901). Experiments in Plant Hybridization. 
 {\it Journal of the Royal Horticultural Society}, 26, 1-32.  

 \r M.B.Mendel (1989). {\it Development of Bayesian Parametric Theory 
 with Application in Control.} PhD Thesis, MIT, Cambridge: MA.

 \r X.L.Meng, W.H.Wong (1996). Simulating Ratios of Normalizing 
 Constants via a Simple Identity: A Theoretical Exploration. 
 {\it Statistica Sinica}, 6, 831-860. 

 \r  A.A.Michelson, E.W.Morley (1887). On the Relative Motion 
 of the Earth and the Luminiferous Ether. 
 {\it American Journal of Physics,} 34, 333--345. 

 \r D.Michie, D.J.Spiegelhalter, C.C.Taylor (1994). {\it Machine Learning, 
  Neural and Statistical Classification.} Ellis Horwood. 

 \r R.E.Michod, B.R.Levin (1988). The Evolution of Sex: An Examination 
 of Current Ideas. Sunderland, MA: Sinauer Associates. 


 \r G.Miller (2000). Mental traits as fitness indicators - expanding
 evolutionary psychology's adaptationism. 
 Evolutionary Perspectives on Human Reproductive Behaviour. 
 {\it Annals of the New York Academy of Sciences}, 907, 62-74.


 \r G.F.Miller (2001). {\it The Mating Mind: How Sexual Choice Shaped 
 the Evolution of Human Nature}. London: Vintage.

 \r G.F.Miller, P.M.Todd (1995). The role of mate choice in
 biocomputation: Sexual selection as a process of search, optimization,
 and diversification. In: 
 W. Banzhaf, F.H. Eeckman (Eds.) Evolution and biocomputation: 
 Computational models of evolution (pp. 169-204). Berlin: Springer.


 \r J.Miller (2006). Earliest Known Uses of Some of the Words of 
    Mathematics.\\ {\it http://members.aol.com/jeff570/mathword.html}

 \r  J.Mingers (1995) {\it Self-Producing Systems: 
 Implications and Applications of Autopoiesis.} %and   
 NY: Plenum. %NY: %Press. 

 \r  M.Minoux, S.Vajda (1986). {\it Mathematical Programming.} 
 John Wiley. 

 \r A.Mosleh, V,M,Bier (1996). Uncertainty about Probability: 
 A Reconciliation with the Subjectivist Viewpoint. 
 {\it IEEE Transactions on Systems, Man and Cybernetics,} 
 A, 26, 3, 303-311. 

 \r W.Mueller, F.Wysotzki (1994). Automatic Construction of 
 Decision Trees for Classification. {\it Ann. Oper. Res.} 52, 231-247.   

 \r S.H.Muggleton (2006). Exceeding Human Limits. 
    {\it Nature}, 440/23, 409--410. 

 \r I.L. Muntean (2006). {\it Beyond Mechanics: 
  Principle of Least Action in Maupertuis and Euler.} 
  On line doc., University of California at San Diego.    

 \r J.J.Murphy (1986). {\it Technical Analysis of the Future Markets: 
 A Comprehensive Guide to Trading Methods ans Applications.} 
 NY: New York Institute of Finance. 

 \r T.Mikosch(1998). {\it Elementary Stochastic Calculus with 
  Finance in View.} Singapore: World Scientific. 

 \r L.Nachbin (1965). {\it The Haar Integral.}  
    Van Nostrand. 

 \r L.K.Nash (1974). {\it Elements of Statistical Thermodynamics.} 
  NY: Dover. 

 \r R.B.Nelsen (2006, 2nd ed.). {\it An Introduction to Copulas.}
    NY: Springer. 

 \r E.Nelson (1987). {\it Radically Elementary Probability Theory.} 
    AM-117. Princeton University Press.  

 \r  W.Nernst (1909). {\it Theoretische Chemie vom Standpunkte der 
 Avogadroschen Regel und der Thermodynamik.} Stuttgart: F.Enke.  

 \r M.C.Newman, C.Strojan (1998). 
 {\it Risk Assessment: Logic and Measurement.} CRC. 

 \r N.Y.Nikolaev, H.Iba (2001). Regularization Approach to Inductive 
  Genetic Programming. {\it IEEE Transactions on Evolutionary Computation}, 
  5, 4, 359-375. Recombinative Guidance. 

 \r N.Y.Nikolaev, H.Iba (2006). {\it Adaptive Learning of Polynomial 
 Networks.} Genetic and Evolutionary Computation. NY: Springer.  

 \r W.Noeth (1995). {\it Handbook of Semiotics.} 
 Indiana University Press.  

 \r  E.Noether (1918). Invariante Varlationsprobleme. 
 {\it Nachrichten der K\"{o}nighche Gesellschaft der Wissenschaften 
 zu G\"{o}ttingen.} 235--257. 
 Translated: {\it Transport Theory and Statistical Physics,} 
 1971, 1, 183--207.  

 \r J.H.Noseworthy, G.C.Ebers, M.K. Vandervoort, R.E.Farquhar, 
    E.Yetisir, R.Roberts (1994). The impact of blinding on 
    the results of a randomized, placebo-controlled multiple 
    sclerosis clinical trial. {\it Neurology,} 44, 16-20. 

 \r M.F.Ochs, R.S.Stoyanova, F.Arias-Mendoza, T.R.Brown (1999). 
    A New Methods for Spectral Decomposition Using  a Bilinear 
    Bayesian Approach. {\it J.of Magnetic Resonance }, 137, 161-176. 

 \r K.Olitzky edt. (2000). {\it Shemonah Perakim: 
 A Treatise on the Soul by Moshe ben Maimon.} URJ Press.  

 \r D.Ormoneit, V.Tresp (1995). Improved Gaussian Mixtures 
 Density Estimates Using Bayesian Penalty Terms and Network Averaging. 
 {\it Advances in Neural Information Processing Systems 8}, 
 542--548. MIT. 

 \r R.H.J.M. Otten, L.P.P.P. van Ginneken (1989).
 {\it The Annealing Algorithm}.  Boston: Kluwer.

 \r C.C.Paige, M.A.Saunders (1977). Least Squares Estimation of 
   Discrete Linear Dynamic Systems using Orthogonal Transformations. 
   {\it Siam J. Numer. Anal.} 14,2, 180-193.  

 \r A.Pais (1988). {\it Inward Bound: Of Matter and Forces in the 
    Physical World.} Oxford University Press. 

 \r C.D.M.Paulino,  C.A.B.Pereira (1992). 
 Bayesian Analysis of Categorical Data Informatively Censored. 
 {\it Communications in Statistics - Theory and Methods}, 21, 2689-705.

 \r C.D.M.Paulino, C.A.B.Pereira (1995). Bayesian Methods for 
 Categorical Data under Informative General Censoring. 
 {\it Biometrika}, 82,2, 439-446.

 \r J.Pearl (2000). 
  {\it Caysality: Models, Reasoning, and Inference.''}
  Cambridge University Press.

 \r J.Pearl (2004). {\it Simpson's Paradox: An Anatomy.} 
    Rech.Rep. Cognitive Systems Lab., Computer Science Dept., 
    Univ.of California at Los Angeles.  

 \r C.S.Peirce (1883). {\it The John Hopkins Studies in Logic.} 
  Boston: Little, Brown and Co. 

 \r C.S.Peirce, J.Jastrow (1885). On small Differences of Sensation.
  {\it Memirs of the National Academy of Sciences}, 3 (1884), 75-83. 
  Also in Kloesel (1993), v.5 (1884-1886), p.122-135. 
 
 \r C.A.B.Pereira, D.V.Lindley (1987). Examples Questioning the use 
 of Partial Likelihood. {\it The Statistician}, 36, 15--20. 

 \r  C.A.B.Pereira, J.M.Stern (1999a).  
 A Dynamic Software Certification and Verification Procedure. 
 Proc. {\it ISAS-99, Int.Conf.on Systems Analysis and Synthesis,} 
 2, 426--435. 

 \r  C.A.B.Pereira, J.M.Stern, (1999b). Evidence and Credibility:
 Full Bayesian Significance Test for Precise Hypotheses.
 {\it Entropy Journal}, 1, 69--80.

 \r C.A.B.Pereira, J.M.Stern (2001a). Full Bayesian Significance
 Tests for Coefficients of Variation. In: George, E.I. (Editor). 
 Bayesian Methods with Applications to Statistics, 391-400. 
 Monographs of Official Statistics, EUROSTAT.    

 \r C.A.B.Pereira,  J.M.Stern (2001b). Model Selection: Full
 Bayesian Approach. {\it Environmetrics} 12, (6), 559-568. 

 \r C.A.B.Pereira, J.M.Stern (2005). 
 {\it Infer\^{e}ncia Indutiva com Dados Discretos: 
 Uma Vis\~{a}o Genuinamente Bayesiana.} 
 COMCA-2005. Chile: Universidad de Antofagasta. 

 \r C.A.B.Pereira, S.Wechsler (1993). On the Concept 
 of $p$-value. {\it Brazilian Journal of Probability and 
 Statistics}, 7, 159--177.  

 \r C.A.B.Pereira, M.A.G.Viana (1982). 
 {\it Elementos de Infer\^{e}ncia Bayesiana.} 5o Sinape, S\~{a}o Paulo. 

 %\r C.A.B.Pereira, S.Wechsler, J.M.Stern (2007). 
 %Can a Significance Test be Genuinely Bayesian? 
 %Submitted. 

 \r P.Perny, A.Tsoukias (1998).
 {\it On the Continuous Extension of a Four Valued Logic for
 Preference Modelling.} IPMU-98, 302--309.
 7th Conf. on Information Processing and Management of Uncertainty 
 in Knowledge Based Systems. Paris, France. 
 
 \r J.Perrin (1903). {\it Trait\'{e} de Chimie Physique}. 
    Paris: Gauthier-Villars. 

 \r J.Perrin (1906). La discontinuit\'{e} de la Mati\`{e}re. 
  {\it Revue de Mois,} 1, 323-343.  
 
 \r J. B. Perrin (1909). Mouvement Brownien et R\'{e}alit\'{e} 
 Mol\'{e}culaire. {\it Annales de Chimie et de Physiqe}, VIII 18, 5-114.  
 also in p.171-239 of Perrin (1950). 
 Translation: Brownian Movement and Molecular Reality, 
 London: Taylor and Francis. 

 \r J.B.Perrin (1913). {\it Les Atomes}. Paris: Alcan. 
 Translation: {\it Atoms.} NY: Van Nostrand. 

 \r J.Perrin (1950). {\it Oeuvres Scientifiques}. Paris: CNRS. 

 \r G.C.Pflug (1996). {\it Optimization of Stochastic Models: The
 Interface Between Simulation and Optimization}. Boston: Kluwer.  

 \r L.Phlips (1995). 
 {\it Competition Policy: A Game-Theoretic Perspective.}
 Cambridge University Press.  

 \r J.Piaget (1975). {\it L'\'{e}quilibration des Structures Cognitives: 
    Probl\`{e}me Central du D\'{e}veloppement.} Paris: PUF.

 \r J.Piaget (1985). {\it Equilibration of Cognitive Structures: 
 The Central Problem of Intellectual Development.} 
 Univ.of Chicago.  

 \r S.D.Pietra, V.Pietra, J.Lafferty (2001). 
 {\it Duality and Auxiliary Functions for Bregman Distances.}  
 Tec.Rep. CMU-CS-01-109R, Carnegie Mellon. 

 \r S.Pissanetzky (1984). {\it Sparse Matrix Technology.} 
  NY: Academic Press. 

 \r M.Planck (1915). Das Prinzip der kleinsten Wirkung. 
 {\it Kultur der Gegenwart}. Also in p.25-41 of Planck (1944). 

 \r M.Planck (1944) Wege zur physikalischen Erkenntnis. 
 Reden und Vortr\"{a}ge. Leipzig: S.Hirzel.  

 \r M.Planck (1937). Religion and Natural Science. 
 Also in Planck (1950).  

 \r M.Planck (1950). Scientific Autobiography and other Papers. 
  London: Williams and Norgate. 

 \r R.J.Plemmons, R.E.White (1990).  Substructuring Methods for Computing 
 the Nullspace of Equilibrium Matrices. 
 {\it SIAM Journal on Matrix Analysis and Applications}, 11, 1-22.

 \r H.A.Pohl (1967). {\it Quantum Mechanics for Science and Engineering.}  
   Englewood Cliffs: Prentice-Hall.  

 \r  K.R.Popper (1959). 
 {\it The Logic of Scientific Discovery.}  NY: Routledge. 

 \r  K.R.Popper (1963). 
 {\it Conjectures and Refutations: The Growth of Scientific Knowledge.}   
 NY: Routledge. 

 \r H.Pulte (1989). 
  Das Prinzip der kleinsten Wirkung und die Kraftkonzeptionen der 
  rationalen Mechanik: Eine Untersuchung zur Grundlegungsproblemematik 
  bei Leonhard Euler, Pierre Louis Moreau de Maupertuis und Joseph Louis 
  Lagrage. {\it Studia Leibnitiana}, sonderheft 19.   

 \r J.R.Quinlan (1986). Induction of Decision Trees.  
  {\it Machine Learning} 1, 221-234.  


 \r H.Rackham (1926). {\it Aristotle, Nicomachean Ethics.} 
 Harvard University Press. 

 \r S.Rahman, J.Symons, D.M.Gabbay J.P. van Bendegem, eds. (2004).  
  {\it Logic, Epistemology, and the Unity of Science}. NY: Springer. 

 \r  W.Rasch (1998). Luhmann's Widerlegung des Idealismus: 
 Constructivism as a two-front war. 
 {\it Soziale Systeme,} 4, 151--161. 

 \r W.Rasch (2000) Niklas Luhmanns Modernity. Paradoxes of
 Differentiation. Stanford Univ.Press. 
 Specially chapter 3 and 4, also published as:  
 W.Rasch (1998). Luhmanns Widerlegung des Idealismus:
 Constructivism as a  Two-Front War. 
 {\it Soziale Systeme,} 4, 151-159; and     
 W.Rasch (1994). In Search of Lyotard Archipelago, or: 
 How to Live a Paradox and Learn to Like It. 
 {\it New German Critique,} 61, 55-75.   

 \r C.R.Reeves (1993). 
 {\it Modern Heuristics for Combinatorial Problems.} 
 Blackwell Scientific.  

 \r C.R.Reeves, J.E.Rowe (2002). {\it Genetic Algorithms - 
 Principles and Perspectives: A Guide to GA Theory.} 
 Berlin: Springer. 

 \r R.Reintjes, A.de Boer, W.van Pelt, J.M.de Groot (2000).  
  Simpson's Paradox: An Example from Hospital Epidemiology. 
  {\it Epidemiology}, 11, 1, 81-83. 

 \r A.Renyi (1961). On Measures of Entropy and Information. 
 {\it Proc. 4-th Berkeley Symp. on Math Sats. and Prob.} V-I, 547-561.  

 \r P.Ressel (1985). DeFinetti Type Theorems: Analytical approach. 
 {\it Annals Probability,} 13, 898--900. 
  
 \r P.Ressel (1987). 
 A Very General De Finetti Type Theorem. In: Viertl (1987). 
 %{\it Probability and Bayesian Statistics.} NY: Plenum. 

 \r P.Ressel (1988). 
 Integral Representations for Distributions of Symmetric Processes. 
 {\it Probability Theory and Related Fields,} 79, 451--467. 

 \r R.J.Richards (1989). {\it Darwin and the Emergence of Evolutionary 
 Theories of Mind and Behavior.} University Of Chicago Press.  

 \r C.J.van Rijsbergen (2004). {\it The Geometry of Information 
    Retrieval.} Cambridge University Press. 

 \r B.D.Ripley (1987). {\it Stochastic Simulation.} NY: Wiley. 


 \r J.Rissanen (1978). Modeling by Shortest Data Description. 
 {\it Automatica,} 14, 465--471. 

 \r J.Rissanen (1989). {\it Stochastic Complexity in Statistical 
  Inquiry.} NY: World Scientific. 

 \r A.M.Robert (2003). {\it Nonstandard Analysis.} Mineola: Dover. 

 \r C.P.Robert (1996). Mixture of Distributions: Inference and 
 Estimation. in Gilks et al. (1996). 

 \r R.Robertson (2001). One, Two, Three, Continuity. C.S.Peirce 
    and the Nature of the Continuum. {\it Cybernetics \& Human 
    Knowing,} 8, 7-24. 

 %\r G.S.Rogers (1980). {\it Matrix Derivatives}. Lecture Notes in  
 %Statistics Vol. 2. Basel: Marcel Dekker.  

 \r V.Ronchi  (1970). {\it Nature of Light: An Historical Survey.} 
  Harvard Univ. Press.  

 \r  H.Rouanet, J.M.Bernard, M.C.Bert, B.Lecoutre, M.P.Lecoutre,
 B.Le Roux (1998). {\it New Ways in Statistical Methodology. From
 Significance Tests to Bayesian Inference.} Berne: Peter Lang. 

 \r D.J.Rose (1972) {\it Sparse Matrices and Their Applications.} 
    NY: Springer. 

 \r D.J.Rose, R.A.Willoughby (1972). {\it Sparse Matrices.} 
    NY: Plenum Press. 

 \r L.Rosenfeld (2005). {\it Classical Statistical Mechanics.} 
  S\~{a}o Paulo: CBPF - Livraria da F\'{\i}sica. 

 \r R.Royall (1997). {\it Statistical Evidence:
 A Likelihood Paradigm}. London: Chapman \& Hall.

 \r E.Rubin (1915). {\it Visuell wahrgenommene Figuren}. 
    Copenhagen: Cyldenalske Boghandel. 

 \r D.B.Rubin (1978). Bayesian Inference for Causal Effects: 
  The Role of Randomization. {\it The Annals of Statistics,} 
  6, 34-58. 

 \r D.Rubin, D.Thayer (1982). EM Algorithm for ML Factor Analysis. 
  {\it Psychometrika,} 47, 1, 69-76.   

 \r H.Rubin (1987). A Weak System of Axioms for ``Rational'' 
 Behaviour and the Non-Separability of Utility from Prior. 
 {\it Statistics and Decisions}, 5, 47--58. 

 \r R.Y.Rubinstein, D.P.Kroese (2004). {\it The Cross-Entropy Method: 
  A Unified Approach to Combinatorial Optimization, Monte-Carlo
  Simulation and Machine Learning.} NY: Springer. 

 \r C.Ruhla (1992). {\it The Physics of Chance: From Blaise Pascal to 
    Niels Bohr.} Oxford University Press. 

 \r S.Russel (1988). Machine Learning: The EM Algorithm. 
 Unpublished note. 

 \r S.Russell (1998). {\it The EM Algorithm.} 
 On line doc, Univ. of California at Berkeley.   

 \r Ruta v. Breckenridge-Remy Co., USA, 1982.

 \r A.I.Sabra (1981). {\it Theories of Light: From Descartes to Newton.} 
  Cambridge University Press. 

 \r R.K.Sacks, H.Wu (1977). 
  {\it Genearl Relativity for Mathematicians.} NY: Springer. 

 \r L.Sadun (2001). 
  {\it Applied Linear Algebra: The Decoupling Principle.} 
  NY: Prentice Hall. 

 \r Sakamoto,Y. Ishiguro,M. Kitagawa,G. (1986). {\it Akaike Information 
 Criterion Statistics.} Dordrecht: Reidel - Kluwer. 

 \r V.H.S.Salinas-Torres, C.A.B.Pereira, R.C.Tiwari (1997). 
 Convergence of Dirichlet Measures Arising in Context of Bayesian Analysis 
 of Competing Risks Models. {\it J. Multivariate Analysis}, 62,1, 24-35.

 \r V.H.S.Salinas-Torres, C.A.B.Pereira, R.C.Tiwari (2002). Bayesian
 Nonparametric Estimation in a Series System or a Competing-Risks Model.
 {\it J.of Nonparametric Statistics}, 14,4, 449-58.

 \r A. Sangiovanni-Vincentelli, L.O. Chua (1977).
 An Efficient Heuristic Cluster Algorithm for Tearing Large-Scale Networks. 
 {\it IEEE Transactions on Circuits and Systems}, 24, 709-717.

 \r L.Santaella (2002). {\it Semi\'{o}tica Aplicada.} 
    S\~{a}o Paulo: Thomson Learning. 

 \r G.de Santillana (1955). {\it The Crime of Galileo}. 
  University of Chicago Press.  

 \r L.A.Santalo (1976). {\it Integral Geometry and Geometric 
 Probability.} 
 %Encyclopedia of Mathematics and its Applications, 1. 
 London: Addison-Wesley.  

 \r  L.J.Savage (1954): {\it The Foundations of Statistics.}  
 Reprint 1972. NY: Dover.

 \r L.J.Savage (1981). {\it The writings of Leonard Jimmie Savage: 
 A memorial selection.} Institute of Mathematical Statistics. 

 \r J.D.Schaffer (1987). Some Effects of Selection Procedures on 
 Hyperplane Sampling by Genetic Algorithms. 
 p. 89-103 in L.Davis (1987). 

 \r J.M.Schervich (1995). {\it Theory of Statistics.} Berlin, Springer. 

 \r  M.Schlick (1920). Naturphilosophische Betrachtungen \"{u}ber 
 das Kausalprintzip. {\it Die Naturw issenschaften}, 8, 461-474. 
 Translated as, Philosophical Reflections on the Causal Principle, 
 ch.12, p.295-321, v.1 in M.Schlick (1979).    

 \r M.Schlick (1979). Philosophical Papers. Dordrecht: Reidel. 

 \r A.Schopenhauer (1818, 1966). 
  {\it The World as Will and Representation.} NY: Dover. 

 \r E.Schr\"{o}dinger (1926). 
  Quantisierung als Eigenwertproblem.  
  (Quantisation as an Eigenvalue Problem). 
  {\it Annalen der Physic}, 489, 79-79. 
  {\it Physical Review}, 28, 1049-1049. 

 \r E.Schr\"{o}dinger (1945). {\it What Is Life?} 
  Cambridge University Press.  
 
 \r G.Schwarz (1978). Estimating the Dimension of a Model. 
 {\it Ann. Stat.}, 6, 461-464. 

 \r  L.Segal (2001). {\it The Dream of Reality. 
 Heintz von Foerster's Constructivism.}  NY: Springer. 

 \r C. Sechen, K. Lee (1987).  An Improved Simulated Annealing Algorithm 
 for Row-Based Placement. {\it Proc. IEEE International Conference on 
 Computer-Aided Design}, 478-481.

 \r G.Shafer (1982),  Lindley's Paradox. %(with comments). 
 {\it J. American Statistical Assoc.}, 77, 325--51. 
 %Association

 \r  G.Shafer, V.Vovk (2001). {\it Probability and Finance, 
  It's Only a Game!} NY: Wiley. 

 \r B.V.Shah, R.J.Buehler, O.Kempthorne (1964). 
 Some Algorithms for Minimizing a Function of Several Variables. 
 {\it J. Soc. Indust. Appl. Math.} 12, 74--92.  

 \r J.Shedler, D.Westen (2004). Dimensions of Personality Pathology: 
 An Alternative to the Five-Factor Model. 
 {\it American Journal of Psychiatry}, 161, 1743-1754. 

 \r J.Shedler, D.Westen (2005). Reply to T.A.Widiger, T.J.Trull.      
 A Simplistic Understanding of the Five-Factor Model
 {\it American J.of Psychiatry}, 162,8, 1550-1551.  

 \r R.Shibata (1981). An Optimal Selection of Regression Variables. 
 {\it Biometrika,} 68, 45--54. 


 \r G.Shwartz (1978). Estimating the Dimension of a Model. 
 {\it Annals of Statistics,} 6, 461--464. 

 \r H.A.Simon (1996). {\it The Sciences of the Artificial}. 
  MIT Press. 

 \r E.H.Simpson (1951). The Interpretation of Interaction in
  Contingency Tables. {\it Journal of the Royal Statistical Society}, 
  Ser.B, 13, 238-241. 

 \r P.J.Smith, E.Gunel (1984). Practical Bayesian Approaches to the 
 Analysis of 2x2 Contingency Table with Incompletely Categorized Data. 
 {\it Communication of Statistics - Theory and Methods}, 13, 1941-63.

 \r G.M.Souza, A.G.Manzatto (2000). {\it Hierarchquia Auto-Organizada 
  em Sistemas Biol\'{o}gicos.} p.153-173 in D'Otaviano and Gonzales (2000).  

 \r J.C.Spall (2003). {\it Introduction to Stochastic Search and 
 Optimization.} Hoboken: Wiley. 
 
 \r M.D.Springer (1979). 
 {\it The Algebra of Random Variables.} NY: Wiley. 

 \r F.Steier, edt. (1991) {\it Research and Reflexivity.} 
    SAGE Publications. 

 \r M.Stephens (1997). {\it Bayesian Methods for Mixtures of 
 Normal Distributions.} %Ph.D. Thesis, 
 Oxford University.   

 \r J.Stenmark, C.S.P.Wu (2004). Simpsons Paradox, Confounding Variables 
  and Insurance Ratemaking. 

 \r   C.Stern (1959). Variation and Hereditary Transmission.  
 {\it Proceedings of the American Philosophical Society}, 103, 2, 183-189. 

 \r J.M.Stern  (1992). Simulated Annealing with a Temperature 
 Dependent Penalty Function. {\it ORSA Journal on Computing,} 
 4, 311-319. 

 \r J.M.Stern (1994). {\it Esparsidade, Estrutura, Estabilidade 
    e Escalonamento em \'{A}lgebra Linear Computacional.}  
    Recife: UFPE, IX Escola de Computa\c{c}\~{a}o. 
 
 \r J.M.Stern (2001) The Full Bayesian Significant Test for the 
  Covariance Structure Problem. 
 Proc. {\it ISAS-01, Int.Conf.on Systems Analysis and Synthesis,} 
 7, 60-65. 

 \r J.M.Stern (2003a). 
  Significance Tests, Belief Calculi, and Burden of Proof in 
  Legal and Scientific Discourse. Laptec-2003, 
  {\it Frontiers in Artificial Intelligence and its Applications,}    
  101, 139--147.     

 \r J.M.Stern (2004a). Paraconsistent Sensitivity Analysis for 
 Bayesian Significance  Tests. SBIA'04,   
 {\it Lecture Notes Artificial Intelligence,} %in LNAI, 
 3171, 134--143. 

 \r J.M.Stern (2004b). Uninformative Reference Sensitivity in 
 Possibilistic Sharp Hypotheses Tests. MaxEnt 2004, 
 %24th International Workshop on Bayesian Inference 
 %and Maximum Entropy Methods in Science and Engineering. 
 {\it American Institute of Physics Proceedings}, 735, 581--588.  

 \r J.M.Stern (2005).  
  Cognitive Constructivism, 
  Eigen--Solutions, and Sharp Statistical Hypotheses. 
  Proceedings of FIS-2005, 61, 1--23. Basel: MDPI. 
  To appear in: {\it Cybernetics and Human Knowing.}   

 \r J.M.Stern (2006a). Cognitive Constructivism and Language. 
 Tech.Rep. MAC-IME-USP-2006-02. 
 To appear in: {\it Cybernetics and Human Knowing.}   

 \r J.M.Stern (2006b). 
 Decoupling, Sparsity, Randomization, and Objective Bayesian Inference. 
 Tech.Rep. MAC-IME-USP-2006-07.  

 \r J.M.Stern (2006c). Language, Metaphor and Metaphysics: 
  The Subjective  Side of Science. Tech.Rep. MAC-IME-USP-2006-09.  

 \r J.M.Stern, C.O.Ribeiro, M.S.Lauretto, F.Nakano (1998). REAL:
 Real Attribute Learning Algorithm. {\it Proc. ISAS/SCI-98} 2, 315--321.  


 \r J.M.Stern, S.A.Vavasis (1994). 
  Active Set Algorithms for Problems in Block Angular Form. 
  {\it Computational and Applied Mathemathics}, 12, 3, 199-226. 

 \r J.M.Stern, S.A.Vavasis (1993).  
  Nested Dissection for Sparse Nullspace Bases. 
  {\it SIAM Journal on Matrix Analysis and Applications,} 14, 3, 766-775. 

 \r  J.M.Stern, S.Zacks (2002). Testing  Independence %the 
 of Poisson Variates under the Holgate Bivariate Distribution. 
 The Power of a New Evidence Test. {\it Statistical and
 Probability Letters}, 60, 313--320. 

 \r J.M.Stern, S.Zacks (2003). 
  {\it Sequential Estimation of Ratios, with Applications to 
  Bayesian Analysis.} Tech. Rep. RT-MAC-2003-10.  

 \r S.M.Stigler (1978). Mathematical Statistics in the Early States. 
 {\it The Annals of Statistics,} 6, 239-265. 

 \r S.M.Stigler (1986). {\it The History of Statistics: The Measurement
    of Uncertainty before 1900}.  Harvard Univ.Press. 

 \r M.St\"{o}ltzner (2003). The Principle of Least Action as the
 Logical Empiricist's Shibboleth. 
 {\it Studies in History and Philosophy of Modern Physics}, 34, 285-318.   

 \r R.D.Stuart (xxxx). {\it An Introduction to Fourier Analysis}. 
 London: Methuen.  


 \r L Szilard (1929). \"{U}ber die Entropieverminderung in einem
  Thermodynamischen System bei Eingriffen Intelligenter Wesen.  
  {\it Zeitschrift f\"{u}r Physik}, 53, 840.

 \r M.Teboulle (1992). Entropic Proximal Mappings with Applications 
 to Nonlinear Programming. {\it Mathematics of operations Research,}  
 17, 670-690. 

 \r C.J.Thompson (1972). {\it Mathematical Statistical Mechanics.} 
  Princeton University Press. 
 
 \r G.L.Tian, K.W.Ng, Z.Geng (2003). Bayesian Computation for
 Contingency Tables with Incomplete Cells-Counts. 
 {\it Statistica Sinica}, 13, 189-206.


 \r W.Tobin (1993). Toothed Wheels and Rotating Mirrors. 
 {\it Vistas in Astronomy}, 36, 253-294. 

 \r S.Tomonaga (1962). {\it Quantum Mechanics.  
  V.1 Old Quantum Theory; V.2, New quantum theory.} 
  North Holland and Interscience Publishers.   


 \r C.A. Tovey (1988). {\it Simulated Simulated Annealing}.
 In Johnson (1988).


 \r M.Tribus, E.C.McIrvine (1971). Energy and Information.  
 {\it Scientific American}, 224, 178-184.  

 \r C.Tsallis (2001). Nonextensive Statistical Mechanics and 
 Termodynamics: Historical Background and Present Status. 
 p. 3-98 in Abe and Okamoto (2001) 

 \r S.M.Ulam (1943). What is a Measure? 
  {\it The American Mathematical Monthly.} 50, 10, 597-602. 

 \r S.Unger, F.Wysotzki (1981). 
  {\it Lernfachige Klassifizirungssysteme.} Berlin: Akademie Verlag. 

 \r J.Uffink (1995). The Constraint Rule of the Maximum Entropy 
 Principle. {\it Studies in the History and Philosophy of Modern 
 Physics,} 26B, 223-261. 

 \r J.Uffink (1996). Can the Maximum Entropy principle be Explained as 
 a Consistency Requirement?. {\it Studies in the History and Philosophy of 
 Modern Physics,} 27, 47-79.  

 \r V.N.Vapnik (1995). {\it The Nature of Statistical Learning Theory.} 
 NY: Springer.   

 \r V.N.Vapnik (1998). {\it Statistical Learning Theory: Inference 
 for Small Samples.} NY: Wiley.  

 \r M.Vega Rod\'{\i}guez, (1998). La Actividad Metaf\'{o}rica: 
  Entre la Raz\'{o}n Calculante y la Raz\'{o}n Intuitiva. 
  {\it Es\'{e}culo, Revista de estudios literarios}. 
  Madrid: Universidad Complutense.   

 \r M.Viana (2003). {\it Symmetry Studies, An Introduction.} 
 Rio de Janeiro: IMPA.  
 %- Instituto de Matem\'{a}tica Pura e Aplicada. 

 \r R.Viertl (1987). 
 {\it Probability and Bayesian Statistics.} NY: Plenum. 

 \r M.Vidyasagar (1997). {\it A Theory of Learning and Generalization.} 
 Springer, London. 

 \r H.M.Voigt, H.Muehlenbein, H.P.Schwefel (1989). 
 {\it Evolution and Optimization.} 
 Berlin: Akademie Verlag. 
 
 \r  H.A.van der Vorst, P.van Dooren, eds. (1990). 
    {\it Parallel Algorithms for Numerical Linear Algebra.} 
    Amsterdam: North-Holland.   

 \r Hugo de Vries (1889). {\it Intracellular Pangenesis Including 
 a paper on Fertilization and Hybridization}.   
 Translated by C.S.Gager (1910). Chicago: The Open Court Publishing Co.   

 \r H.de Vries (1900). 
 Sur la loi de disjonction des hybrides. 
 {\it Comptes Rendus de l'Academie des Sciences}, 130, 845-847. 
 Translated as  Concerning the law of segregation of hybrids. 
 {\it Genetics}, (1950), 35, 30-32. 

 \r S.Walker(1986). A Bayesian Maximum Posteriori Algorithm for
 Categorical Data under Informative General Censoring. 
 {\it The Statistician}, 45, 293-8.

 \r C.S.Wallace, D.M.Boulton (1968), An Information Measure for
 Classification. {\it Computer Journal}, 11,2, 185-194. 

 \r C.S.Wallace, D.Dowe (1999). Minimum Message Length and 
 Kolmogorov Complexity. {\it Computer Journal}, 42,4, 270-283. 

 \r W.A.Wallis (1980). The Statistical Research Group, 1942-1945.   
 {\it Journal of the American Statistical Association}, 75, 370, 320-330. 

 \r  S.Wechsler, L.G.Esteves, A.Simonis, C.Peixoto (2005). 
 Indiference, Neutrality and Informativeness: 
 Generalizing the Three Prisioners Paradox. 
 {\it Synthese}, 143, 255-272. 

 \r  R.L.Weil, P.C.Kettler (1971).
 Rearranging Matrices to Block Angular Form for Decomposition Algorithms. 
 {\it Management Science}, 18, 1, 98-108.

 \r  E.Wenger, R.Pea, J.S.Brown, C.Heath (1999). 
 {\it Communities of Practice: Learning, Meaning, and Identity.} 
 Cambridge Univ. Press. 

 \r T.A.Widiger, E.Simonsen (2005). Alternative Dimensional Models of
  Personality Disorder: Finding a Common Ground. 
  {\it J.of Personality Disorders}, 19, 110-130

 \r F.W.Wiegel (1986). {\it Introduction to Path-Integral Methods in 
 Physics and Polymer Science.} Singapore: World Scientific. 

 \r E.P.Wigner (1960).  
 The Unreasonable Effectiveness of Mathematics in the Natural Sciences.  
 {\it Communications in Pure and Applied mathematics,} 13,1. 
 Also in ch.17, p.222-237 of Wigner (1967). 

 \r E.P.Wigner (1967). {\it Symmetries and Reflections.} 
 Bloomington: Indiana University Press.  

 \r D.Williams (2001) {\it Weighing the Odds.} 
 Cambridge Univ. Press.  

 \r R.C.Williamson (1989). {\it Probabilistic Arithmetic.} %PhD Thesis, 
 Univ. of Queensland.  

 \r S.S.Wilks (1962). {\it Mathematical Statistics.}  NY: Wiley. 

 \r R.L.Winkler (1975). 
 {\it Statistics: Probability, Inference, and Decision.}  
 Harcourt School. 

 \r  T.Winograd, F.Flores (1987).             
  {\it Understanding Computers and Cognition: 
  A New Foundation for Design} 
  NY: Addison-Wesley. 
 \r H.Weyl (1952). {\it Symmetry.} Princeton Univ. Press. 

 \r D.A.Wismer, ed. (1971). {\it Optimization Methods for Large-Scale 
    Systems with Applications.} NY: McGaw-Hill. 

 \r S.R. White (1984). Concepts of Scale in Simulated Annealing.
 {\it American Institute of Physics Conference Proceedings}, 122, 261-270.

 \r   R.G.Winther (2000). Darwin on Variation and Hereditarity. 
    {\it Journal of the History of Biology}, 33, 425-455. 

 \r  L.Wittgenstein (1921). 
 {\it Tractatus Logico Philosophicus}  
 (Logisch-Philosophische Abhandlung). 
 (Ed.1999) NY: Dover.  

 \r L.Wittgenstein (1953). 
  {\it Philosophische Untersuchungen.} 
  Philosophical Investigations, english transl. by 
  G.E.M.Anscombe. Oxford: Blackwell. 

 \r W.Yourgrau S.Mandelstam (1979). {\it Variational Principles in 
 Dynamics and Quantum Theory.} NY: Dover. 

 \r L.A.Zadeh (1987). {\it Fuzzy Sets and Applications}.
 NY: Wiley. 

 \r A.Zahavi (1975).  Mate selection: A selection for a handicap.  
 {\it Journal of Theoretical Biology}, 53, 205-214.

 \r  M.Zelleny (1980). {\it Autopoiesis, Dissipative Structures, 
 and Spontaneous Social Orders.}  
 Washington: %AAAS -   
 American Association for the Advancement of Science. 

 \r A.Zellner (1971). {\it Introduction to
  Bayesian Inference in Econometrics.} NY:Wiley.

 \r A.Zellner (1982). Is Jeffreys a Necessarist? 
 {\it American Statistician}, 36, 1, 28-30.  

 \r V.I.Zubov (1983). {\it Analytical Dynamics of Systems of 
  Bodies.} Leningrad Univ.  %ersity. 

 \r M.A.Zupan (1991). Paradigms and Cultures: Some Economic Reasons for 
  Their Stickness. {\it The American Journal of Economics and Sociology},  
  50, 99-104.    

 
\end{small} 
%\end{footnotesize}
%\end{scriptsize} 
\renewcommand{\baselinestretch}{1.1}
\parskip 0.2cm
%\pagebreak  




